Beyond Catoni: Sharper Rates for Heavy-Tailed and Robust Mean Estimation

We study the fundamental problem of estimating the mean of a $d$-dimensional distribution with covariance $\Sigma \preccurlyeq \sigma^2 I_d$ given $n$ samples. When $d = 1$, \cite{catoni} showed an estimator with error $(1+o(1)) \cdot \sigma \sqrt{\frac{2 \log \frac{1}{\delta}}{n}}$, with probability $1 - \delta$, matching the Gaussian error rate. For $d>1$, a natural estimator outputs the center of the minimum enclosing ball of one-dimensional confidence intervals to achieve a $1-\delta$ confidence radius of $\sqrt{\frac{2 d}{d+1}} \cdot \sigma \left(\sqrt{\frac{d}{n}} + \sqrt{\frac{2 \log \frac{1}{\delta}}{n}}\right)$, incurring a $\sqrt{\frac{2d}{d+1}}$-factor loss over the Gaussian rate. When the $\sqrt{\frac{d}{n}}$ term dominates by a $\sqrt{\log \frac{1}{\delta}}$ factor, \cite{lee2022optimal-highdim} showed an improved estimator matching the Gaussian rate. This raises a natural question: Is the $\sqrt{\frac{2 d}{d+1}}$ loss \emph{necessary} when the $\sqrt{\frac{2 \log \frac{1}{\delta}}{n}}$ term dominates? We show that the answer is \emph{no} -- we construct an estimator that improves over the above naive estimator by a constant factor. We also consider robust estimation, where an adversary is allowed to corrupt an $\epsilon$-fraction of samples arbitrarily: in this case, we show that the above strategy of combining one-dimensional estimates and incurring the $\sqrt{\frac{2d}{d+1}}$-factor \emph{is} optimal in the infinite-sample limit.

==> everything_else.tex <==
\section{Catoni Estimator Using Newton's method}
Consider a score function $s$ with
\begin{align*}
    s(x) = 
    \begin{cases}
    \log(1+x + x^2/2) & x \ge 0\\
    -\log(1 - x + x^2/2) & x < 0
    \end{cases}
\end{align*}
We are given samples $X_1, \dots, X_n$ with mean $\mu$ and variance $\sigma^2$. Consider an initial estimate of the mean $\mu$, $\mu_1 = \mu + \eps$ with $|\eps| \lesssim \sigma \sqrt{\frac{\log \frac{1}{\delta}}{n}}$. Consider for parameter $\theta$,
\begin{align*}
    r(\theta) = \frac{1}{\alpha n} \sum_{i=1}^n s(\alpha (X_i - \theta))
\end{align*}
for $\alpha = \sqrt{\frac{2 \log \frac{1}{\delta}}{n(\sigma^2 + \eta^2)}}$. We will compute $r(\mu_1)$. We have
\begin{align*}
     \E[\exp(\alpha n r(\mu_1))] &=  \prod_{i=1}^n \E\left[\exp(s(\alpha (X_i - \mu - \eps))) \right]\\
     &\le \left(1 -\alpha \eps + \frac{\alpha^2}{2} \left(\sigma^2 + \eps^2 \right)\right)^n\\
     &\le \exp\left(-n \alpha \eps + \frac{n \alpha^2}{2} \left(\sigma^2 + \eps^2 \right) \right)
\end{align*}

\section{High dimensional estimation}
\paragraph{Algorithm.} For $Y_1, \dots, Y_n \in \R$, let Catoni($Y_1, \dots, Y_n$) be the Catoni estimate of the samples $Y_1, \dots, Y_n$. Then, for $X_1, \dots, X_n \in \R^d$, find $\wh \mu$ that minimizes 
\[
    \sup_{v \in S^{d-1}} \text{Catoni}\left(v^T(X_1 - \wh \mu), \dots, v^T(X_n - \wh \mu) \right)
\]
XXX BELOW IS SCRATCH:
\begin{lemma}
    The true mean $\mu$ satisfies that with probability $1 - \delta$,
    \[
        \sup_{v \in S^{d-1}} \text{Catoni}\left(v^T(X_1 - \mu), \dots, v^T(X_n - \mu) \right) \le \sqrt{\frac{\Tr(\Sigma)}{n}} + \sqrt{\frac{2 \log \frac{1}{\delta}}{n}}\left(1 + o(1) \right)
    \]
\end{lemma}
\begin{proof}
    The Catoni estimator has the guarantee that for any fixed $v$, with probability $1-\delta$,
    \begin{align*}
        \text{Catoni}\left( v^T (X_i - \mu)\right) \le  \sqrt{v^T \Sigma v} \sqrt{\frac{2\log \frac{2}{\delta}}{n}} \left(1 + O\left(\frac{\log \frac{1}{\delta}}{n} \right) \right)
    \end{align*}
\end{proof}

First note that for our score function, we have, for $v \sim \mathcal N(0, I_d)$,
\begin{align*}
    \E_{v}\left[\exp\left(s\left(\alpha v^T (X_i - \theta) \right) \right) \right] &\le \E_{v} \left[ 1 + \alpha v^T (X_i - \theta) + \frac{\alpha^2}{2} (v^T (X_i- \theta))^2\right]\\
    &= 1 + \frac{\alpha^2}{2} \|X_i -\theta\|^2 \quad \text{since $v^T (X_i - \theta) \sim \mathcal N(0, \|X_i - \theta\|^2)$}\\
    &\le e^{\frac{\alpha^2 \|X_i - \theta\|^2}{2}}
\end{align*}

XXX BEGIN HERE:
First,
\begin{align*}
    \E_{X}\left[\sup_{v \in S^{d-1}}\prod_{i=1}^n e^{s(\alpha v^T (X_i - \theta))} \right] &\le \E_{X}\left[\sup_{v \in S^{d-1}}\prod_{i=1}^n  \left(1 + \alpha v^T (X_i - \theta) + \frac{\alpha^2}{2} (v^T(X_i - \theta))^2 \right)\right]\\
    &\le \E_X\left[\sup_{v \in S^{d-1}} \prod_{i=1}^n e^{\alpha v^T (X_i- \theta) + \frac{\alpha^2}{2} (v^T (X - \theta))^2} \right]\\
    %&= \E_X\left[\sup_{v \in S^{d-1}} e^{\alpha v^T(\sum_i (X_i - \theta)) + \frac{\alpha^2}{2} \sum_{i=1}^n \left(v^T (X_i - \theta) \right)^2\right]
\end{align*}

Interesting thing:
\begin{align*}
    \sup_{v \in S^{d-1}} e^{s(\alpha v^T (X_i - \theta))} = e^{s(\alpha \|X_i - \theta\|)} = 1 + \alpha \|X_i - \theta\| + \frac{\alpha^2}{2} \|X_i - \theta\|^2
\end{align*}
and
\begin{align*}
    \E_{v \sim \mathcal N(0, I_d)}\left[e^{\sign(v^T (X_i - \theta)) \cdot s(\alpha v^T (X_i -\theta))} \right] &= \E_{v} \left[1 + |v^T (X_i - \theta)| + (v^T (X_i - \theta))^2 \right]
\end{align*}
\subsection{Strategy}
First, define $r_v(\theta)$ to be the total score at $\theta \in R^d$ when projected onto $v$. That is
\begin{align*}
    r_v(\theta) = \frac{1}{\alpha n} \sum_{i=1}^n s\left(\alpha \cdot \frac{v}{\|v\|}^T\left(X_i - \theta \right)\right)
\end{align*}
Consider any point $\theta \in \R^d$ ``far enough'' away from the true mean $\mu$. Since it is far enough away, we want to say that with probability $1 - \delta$, $r_{\mu - \theta}(\theta) > 0$. That is, if we project the data onto $\mu - \theta$, the total score at $\theta$ should be bounded away from $0$, since $\theta$ is far from the true mean $\mu$.

We know by the Catoni analysis that this is going to be true for any $\theta$ such that more than $\sqrt{2 \frac{\log \frac{2}{\delta}}{n}}\left(1 + O\left(\frac{\log \frac{1}{\delta}}{n} \right) \right)$ away. So, by a union bound over a net, we can get that for all $\theta$ such that $\|\theta - \mu\| \gtrsim \left(\sqrt{\frac{2 d}{n}} + \sqrt{2 \frac{\log \frac{2}{\delta}}{n}}\right)\left(1 + O\left(\frac{\log \frac{1}{\delta}}{n} \right) \right) $, $r_{\mu - \theta}(\theta) > 0$. This means that the Catoni estimate in every direction is inside this radius so that our $\mu$ satisfies that with probability $1 - \delta$,
\begin{align*}
    \sup_{v \in S^{d-1}} \text{Catoni}\left(v^T(X_1 - \mu), \dots, v^T(X_n - \mu) \right) \lesssim \sqrt{\frac{2 d}{n}} + \sqrt{\frac{2 \log \frac{2}{\delta}}{n}}
\end{align*}

To get tight constants, we need to do more work.

\section{Second Objective function}
Let $\curlyE(\theta, y) = \frac{1}{n \lam} \sum \int \psi(\lam\langle \theta', X_i - y \rangle) d \rho_\theta(\theta')$. We will find $\hat \mu$ by
\[
    \min_{\hat \mu} \sup_\theta \curlyE(\theta, \hat \mu)
\]
Let the true mean be $0$. By the PAC-Bayes inequality, we know that
\[
    \sup_\theta \curlyE(\theta, 0) \le \sqrt{\frac{\Tr(\Sigma)}{n}} + \sqrt{\frac{2\|\Sigma\| \log \frac{2}{\delta}}{n}} := C
\]
Note that $\psi(x)$ is sublinear, and approximated well by $x$ (in fact this seems better than reality for what we're about to do).

Suppose $\curlyE(e_1, 0) = \curlyE(e_2, 0) = C$, and $\curlyE(e_i, 0) = 0$ for all $i \ge 3$. 

\textbf{Claim:} $\sup_\theta \curlyE(\theta, C(e_1 + e_2)) \approx 0$ and $\sup_\theta \curlyE(\theta, y) > C\left(1 - \frac{1}{\sqrt{2}}\right)$ for all $\|y\| < C$.

First, by our linear approximation
\[
    \curlyE(\theta, y) \approx \curlyE(\theta, 0) - \inner{\theta, y}
\]
Also note that
\[
    \curlyE(\theta, 0) \approx C \inner{\theta, e_1+e_2}
\]

So, for any $\theta$,
\begin{align*}
    \curlyE(\theta, e_1 + e_2) &\approx \curlyE(\theta, 0) - C\inner{\theta, e_1 + e_2} \\
    &\approx C \inner{\theta, e_1+e_2} - C \inner{\theta, e_1 + e_2} \approx 0
\end{align*}
%where the maximizer is $\theta = \frac{e_1 + e_2}{\sqrt{2}}$.

Now, for $y$ with $\|y\| < C$, wlog, suppose $\inner{e_1, y} \le \inner{e_2, y}$ and that $\inner{e_1, y} > 0$. Since $\inner{\frac{e_1 + e_2}{\sqrt{2}}, y} \le C$, this condition implies that $\inner{e_1, y} \le C/\sqrt{2}$. Then,
\[
    \curlyE(e_1, y) \approx C \inner{e_1, e_1 + e_2} - \inner{e_1, y} \ge \left(1 - \frac{1}{\sqrt{2}} \right) C
\]

Intuitively, this is saying the $y$ minimizing the objective within the sphere of radius $C$ is at $\frac{e_1 + e_2}{\sqrt{2}} C$.

Maybe the above doesn't work (the linear approximation is bad). Specifically, if you generalize the argument, it seems like it's saying that the minimizer could be as far as $\sqrt{d}$ away, which is not true.

A different type of argument.

\subsection{Maybe this works?}

We know with probability $1 - \delta$, for every $y$ with $\|y\| > C$, $\curlyE(y, y) > 0$. So, can we show that if we move towards $0$, the objective decreases? That is 
\[
    \sup_\theta \curlyE(\theta, (1 - \eps) y) < \sup_\theta \curlyE(\theta, y)
\]
Why might this be true? It seems like for $\theta$ orthogonal to $y$ the objective shouldn't change much as you move, while it should decrease for the directions with positive projection onto $y$.

\begin{lemma}[PAC-Bayes]
    \label{lem:pac_bayes}
    Let $\mu$ be a measure on $\Theta$. For $\delta \in (0, 1)$, with probability at least $1 - \delta$, for every probability measure $\rho$ on $\Theta$,
    \[
        \frac{1}{n} \sum_{i=1}^n \E_{\theta \sim \rho}\left[f(\theta, X_i) \right] \le \E_{\theta \sim \rho} \left[ \log \E_X\left[\exp\left(f(\theta, X) \right) \right]\right] + \frac{D_{KL}(\rho \| \mu) + \log \frac{1}{\delta}}{n}
    \]
\end{lemma}

    Let $\rho_v = \mathcal N(v, \beta^{-1} I_d)$. Let 
     \[
        C := \sqrt{\frac{\Tr(\Sigma)}{n}} + \sqrt{\frac{2 \|\Sigma\| \log \frac{2}{\delta}}{n}}
    \]
    and define 
    \[
        g(v) := \frac{1}{n \lam} \sum_{i=1}^n \E_{\theta \sim \rho_v}\left[ \psi\left(\lam \inner{\theta, X_i - C \theta} \right)\right]
    \]

    Also, our $\psi$ satisfies
    \begin{align}
        -\log(1 - t + t^2/2) \le \psi(t) \le \log(1 + t + t^2/2)
    \end{align}
\subsection{Gaussian case}
Just to understand better, here's what happens for the Gaussian.
The left hand side of the PAC-Bayes inequality is
\begin{align*}
    \frac{1}{n} \sum_{i=1}^n \E_{\theta \sim \rho_v}\left[\lam \inner{\theta, X_i - C \theta} \right] &= \frac{\lam}{n} \sum_{i=1}^n \left(\inner{v, X_i} - C \E_{\theta \sim \rho_v}\left[\|\theta\|^2\right] \right)\\
    &= \frac{\lam}{n} \sum_{i=1}^n \inner{v, X_i - C v} - C \beta^{-1} d
\end{align*}
The first term on the right hand side is
\begin{align*}
    \E_{\theta \sim \rho_v}\left[\log\left(\E_{X}\left[\exp\left(\lam \inner{\theta, X - C \theta} \right) \right] \right) \right] &\le \E_{\theta \sim \rho_v}\left[ \lam^2 \theta^T \Sigma \theta/2 - C \lam \|\theta\|^2 \right]\\
    &= \frac{1}{2} \left(\lam^2 v^T \Sigma v + \lam^2 \beta^{-1} \Tr(\Sigma)\right) - \lam C - \lam C \beta^{-1} d
\end{align*}
So it seems like if you add $\lam C \beta^{-1} d$ to both sides you should get the right thing.
\subsection{The real thing}
\paragraph{Definition.} Let our function of interest be (for our setting of $\lam$ and $\beta$)
\[
    h(v) = g(-v) - C \beta^{-1} d + \lam \frac{C^2}{2} \left[1 + \beta^{-1} (5 + d) + \beta^{-2} d(d+2) \right]
\]
The above function is coming from the fact that the residual term is
\begin{align*}
    C \beta^{-1} d - \frac{\lam}{2} C^2 \E_{\theta \sim \rho_v}\left[\|\theta\|^4\right]
\end{align*}
Here 
\begin{align*}
    \E_{\theta \sim \rho_v}\left[\|\theta\|^4 \right] &= \sum_{i=1}^d \E\left[ \theta_i^4\right] + \sum_{i \neq j}\left[\theta_i^2 \theta_j^2 \right]\\
    &= \sum_{i=1}^d \left( v_i^4 + 6 v_i^2 \beta^{-1} + 3 \beta^{-2}\right) + \sum_{i \neq j}\left(v_i^2 v_j^2 + \beta^{-1} (v_i^2 + v_j^2) + \beta^{-2} \right)\\
    &= \|v\|^4 + 6 \beta^{-1} \|v\|^2 + 3 d \beta^{-2} + (d-1) \beta^{-1} \|v\|^2 + d(d-1) \beta^{-2}\\
    &= 1 + \beta^{-1} (5 + d) + \beta^{-2} d(d+2)
\end{align*}
\begin{lemma}
    Suppose the true mean of the $X_i$'s is $0$. Set 
    \[
        \lam = \sqrt{\frac{2 \log \frac{1}{\delta}}{n \|\Sigma\|}}
    \]
    and
    \[
        \beta = \sqrt{\frac{2 \Tr(\Sigma) \log \frac{1}{\delta}}{\|\Sigma\|}}
    \]
    We have that with probability $1 - \delta$, for every $v \in S^{d-1}$,
    \begin{align*}
        h(v) > 0
    \end{align*}
\end{lemma}
\begin{proof}
     Let $f(\theta, X_i) = \psi(\lam\inner{\theta, X_i - C\theta})$ and let the prior be $\rho_0$. By the PAC-Bayes inequality of Lemma~\ref{lem:pac_bayes} and the property of our $\psi$, we have that with probability $1 - \delta$
    \begin{align*}
        g(v) &\le \frac{1}{\lam} \E_{\theta \sim \rho_v} \left[\log\left(1 + \E_X\left[\lam \inner{\theta, X - C \theta} \right] + \frac{1}{2} \E_X\left[\lam^2 \inner{\theta, X - C \theta}^2 \right]\right) \right] + \frac{\beta + 2 \log \frac{1}{\delta}}{2 n \lam}\\
        &\le \E_X\left[ \inner{\theta, X} \right] - C \E_{\theta \sim \rho_v} \left[\|\theta\|^2 \right] + \frac{\lam}{2}\E_{X, \theta \sim \rho_v} \left[\left(\inner{\theta, X} - C \|\theta\|^2 \right)^2 \right] + \frac{\beta + 2 \log \frac{1}{\delta}}{2 n \lam}\\
        &= -C \left(\|v\|^2 + \beta^{-1} d \right) + \frac{\lam}{2} \left(\E_{X, \theta'}\left[\inner{\theta', X}^2 \right] + C^2\E_{\theta'} \left[\|\theta'\|^4 \right]\right) + \frac{\beta + 2 \log \frac{1}{\delta}}{2n \lam}\\
        &= -C - C \beta^{-1} d + \frac{\lam}{2} \left( \right)
    \end{align*}
\end{proof}

\subsection{Correcting things}
It seems like the above doesn't really work because $\E_{\theta \sim \rho_v}[\inner{\theta, X - C\theta}]$ is not something you can really compute, since $C \theta$ is also random.

The function we should look at instead is
\[
    h(v, \hat \mu) = \frac{1}{n} \sum_{i=1}^n \E_{\theta \sim \rho_v}\left[\psi\left(\inner{\theta, X_i - \hat \mu}\right) \right]
\]
We will now relate $g$ to $h$.
Note that $\psi$ is sublinear, so that $\psi(a - b) \ge \psi(a) - b$ for $b > 0$.
\begin{lemma}
    Let 
    \begin{equation*}
        \psi(t) = 
        \begin{cases}
            t - t^3/6, &-\sqrt{2} \le t \le \sqrt{2}\\
            2 \sqrt{2}/3, &t > \sqrt{2}\\
            -2 \sqrt{2}/3, &t < -\sqrt{2}
        \end{cases}
    \end{equation*}
        We have that $\psi(a - b) \ge \psi(a) - b$ for $b \ge 0$.
\end{lemma}
\begin{proof}
    It suffices to show that $(a - b) - (a - b)^3/6 \ge a - a^3/6 - b$. This is equivalent to showing $(3 a^2 b - 3 a b^2 + b^3)/6 \ge 0$. This seems to be true from plotting.
\end{proof}

\begin{lemma}
    For $v \in S^{d-1}$,
    \begin{align*}
        \frac{1}{n \lam}\sum_{i=1}^n \E_{\theta \sim \rho_v}\left[\psi\left(\lam \inner{\theta, X_i - Cv} \right) \right] \le \frac{1}{n\lam} \sum_{i=1}^n \E_{\theta \sim \rho_v}\left[\psi(\lam \inner{\theta, X_i - C \frac{\theta}{\|\theta\|}}) \right] + C \E_{\theta \sim \rho_v}[\|\theta\|] - C
    \end{align*}    
\end{lemma}
\begin{proof}
    \begin{align*}
        \E_{\theta \sim \rho_v}\left[\psi(\lam \inner{\theta, X_i - C \frac{\theta}{\|\theta\|}}) \right] &= \E_{\theta \sim \rho_v}\left[\psi\left(\lam\left( \inner{\theta, X_i - C v} - C\inner{\theta, \frac{\theta}{\|\theta\|} - v}  \right)\right) \right]\\
        &\ge \E_{\theta \sim \rho_v}\left[\psi\left(\lam\left(\inner{\theta, X_i - C v} \right) \right) - \lam C  \inner{\theta, \frac{\theta}{\|\theta\|} - v}\right] \quad \text{since $\inner{\theta, \frac{\theta}{\|\theta\|} - v} \ge 0$}\\
        &= \E_{\theta \sim \rho_v}\left[\psi\left(\lam\inner{\theta, X_i - C v} \right)  \right] - \lam C \E_{\theta \sim \rho_v}\left[\|\theta\| \right] + \lam C \E_{\theta \sim \rho_v}\left[\inner{\theta, v}\right]\\
        &= \E_{\theta \sim \rho_v}\left[\psi\left(\lam\inner{\theta, X_i - C v} \right)  \right] - \lam C \E_{\theta \sim \rho_v}\left[\|\theta\| \right] + \lam C \quad \text{since $\inner{\theta, v} \sim \mathcal N(\|v\|^2, \beta^{-1} \|v\|^2)$}
    \end{align*} 
    The claim follows.
\end{proof}
\begin{lemma}
    Setting 
    \[
        \lam = \sqrt{\frac{2 \log \frac{1}{\delta}}{n \|\Sigma\|}}
    \]
    and
    \[
        \beta = \sqrt{\frac{2 \Tr(\Sigma) \log \frac{1}{\delta}}{\|\Sigma\|}}
    \]
    we have with probability $1 - \delta$, for every $v \in S^{d-1}$,
    \begin{align*}
        \frac{1}{n \lam} \sum_{i=1}^n  \E_{\theta \sim \rho_v}\left[\psi\left(\lam\inner{\theta, X_i - C \frac{\theta}{\|\theta\|} } \right) \right]
    \end{align*}
\end{lemma}
\begin{proof}
     Let $f(\theta, X_i) = \psi(\lam\inner{\theta, X_i - C\theta})$ and let the prior be $\rho_0$. By the PAC-Bayes inequality of Lemma~\ref{lem:pac_bayes} and the property of our $\psi$, we have that with probability $1 - \delta$, for every $v \in S^{d-1}$,
    \begin{align*}
        &\frac{1}{n \lam} \sum_{i=1}^n  \E_{\theta \sim \rho_v}\left[\psi\left(\lam\inner{\theta, X_i - C \frac{\theta}{\|\theta\|} } \right) \right]\\
        &\le \frac{1}{\lam} \E_{\theta \sim \rho_v}\left[\log\left(1 + \E_X\left[\lam \inner{\theta, X - C \frac{\theta}{\|\theta\|}} \right] + \frac{1}{2} \E_X\left[\lam^2 \inner{\theta, X - C\frac{\theta}{\|\theta\|}}^2 \right]\right) \right] + \frac{\beta + 2 \log \frac{1}{\delta}}{2 n \lam}\\
        &\le \E_X\left[\inner{\theta, X} \right] - C \E_{\theta \sim \rho_v}\left[ \|\theta\| \right] + \frac{\lam}{2} \left(\E_{X, \theta \sim \rho_v}\left[\inner{\theta, X}^2 \right] + C^2 \E_{\theta \sim \rho_v}\left[\|\theta\|^2 \right] \right) + \frac{\beta + 2 \log \frac{1}{\delta}}{2 n \lam}\\
    \end{align*}
    First, $\E_X\left[\inner{\theta, X} \right] = 0$ since $\E[X] = 0$. Now, 
    \begin{align*}
        \E_{X, \theta \sim \rho_v}\left[\inner{\theta, X}^2 \right] &=\E_{X}\left[\inner{v, X}^2 \right] + \frac{\E_X[\|X\|^2]}{\beta}\\
        &\le \|\Sigma\| + \frac{\Tr(\Sigma)}{\beta}
    \end{align*}
    Also,
    \begin{align*}
        \E_{\theta \sim \rho_v}\left[ \|\theta\|^2 \right] = \|v\|^2 + \beta^{-1} d = 1 + \beta^{-1} d
    \end{align*}
    So, for our setting of $\beta$ and $\lam$,
    \begin{align*}
        \frac{1}{n \lam} \sum_{i=1}^n  \E_{\theta \sim \rho_v}\left[\psi\left(\lam\inner{\theta, X_i - C \frac{\theta}{\|\theta\|} } \right) \right] &\le -C \E_{\theta \sim \rho_v}\left[\|\theta\| \right] + \frac{\lam C^2}{2}\left(1 + \beta^{-1} d \right) + \sqrt{\frac{\Tr(\Sigma)}{n}} + \sqrt{2 \|\Sigma\| \frac{\log \frac{1}{\delta}}{n}}
    \end{align*}
\end{proof}
\begin{corollary}
    With probability $1 - \delta$, for every $v \in S^{d-1}$
    \begin{align*}
        \frac{1}{n \lam} \sum_{i=1}^n \E_{\theta \sim \rho_v}\left[\psi \left(\lam \inner{\theta, X_i - C v} \right) \right] \le -C + \frac{\lam C^2}{2}(1 + \beta^{-1} d) + \sqrt{\frac{\Tr(\Sigma)}{n}} + \sqrt{2\|\Sigma\| \frac{\log \frac{1}{\delta}}{n}} 
    \end{align*}
\end{corollary}

So it seems like things are fine as long as 
\begin{align*}
    \frac{\lam C}{2} ( 1 + \beta^{-1} d) = o(1)
\end{align*}
The above is
\begin{align*}
    C \sqrt{\frac{2 \log \frac{1}{\delta}}{n \|\Sigma\|}} \left(1 + \sqrt{\frac{\|\Sigma\|}{2 \Tr(\Sigma) \log \frac{1}{\delta}}} d\right)
\end{align*}
This is saying things are fine as long as
\begin{align*}
    C = o\left(\frac{\sqrt{ \Tr(\Sigma) n}}{d} \right)
\end{align*}
Since we want to set $C \approx \sqrt{\frac{\Tr(\Sigma)}{n}} + \sqrt{\frac{2 \|\Sigma\| \log \frac{1}{\delta}}{n}}$, this is true when
$d = o(n)$ and $\log \frac{1}{\delta} = o(n)$, which seems reasonable (XXX This was wrong. It only works for things that are *basically* spherical. But maybe this is ok XXX). Then, we obtain the following.
\begin{lemma}\label{lem:hvCv}
    For $\Sigma = I$ and $n \gg \Tr(\Sigma), n \ll \log \frac{1}{\delta}$, let
    \begin{align*}
        C = \left(\sqrt{\frac{\Tr(\Sigma)}{n}} + \sqrt{2 \|\Sigma\| \frac{\log \frac{1}{\delta}}{n}}\right)(1+o(1)) \quad \text{and} \quad \beta = \sqrt{\frac{2 \Tr(\Sigma) \log \frac{1}{\delta}}{\|\Sigma\|}}
    \end{align*}
    and let $\rho_v = \mathcal N(v, \beta^{-1} I_d)$. Let
    \[
        h(v, \hat \mu) = \frac{1}{n \lam} \sum_{i=1}^n \E_{ \theta \sim \rho_v}\left[\psi\left(\lam\inner{-\theta, X_i - \hat \mu} \right) \right] 
    \]
    Then, we have that with probability $1 - \delta$, for every $v \in S^{d-1}$,
    \[
        h(v, C v) \ge 0
    \]
\end{lemma}


Now, we want to show that for $\hat \mu$ strictly outside the shell of radius $C$, if we project $\hat \mu$ on to the shell, $h$ in *any* direction can only decrease or not change, and will decrease for directions with some projection onto $\hat \mu$.

To establish this, we need some facts.

Note that $h(v, Cv) \ge 0$ and $h(-v, -Cv) \ge 0$ so that $h(v, -Cv) \le 0$. This means that $h(v, t v) = 0$ for some $-C \le t \le C$. Also, for $a \ge C$, $h(v, a v)$ should increase in a and $h(v, -av)$ should decrease in $a$.


\begin{lemma}
    Suppose $a > b$. We have that 
    \[
        h(v, av) > h(v, bv)
    \]
\end{lemma}
\begin{proof}
    Let's look at the summand on the LHS.
    \begin{align*}
        \E_{\theta \sim \rho_v}\left[\psi\left(\lam\inner{-v, X_i - av} \right) \right] &= 
    \end{align*}
\end{proof}

Let $\wh{w}_{\wh{\mu}}$ be $\text{argsup}_{w} h(w, \wh{\mu})$.  We want to show that $\inner{\wh{w}_{\wh{\mu}}, \wh{\mu}} > 0$ for all $\norm{\wh{\mu}} > C$.  Can we show that, for any $w \perp \wh{\mu}$ and $\alpha > 0$
\[
h(w + \alpha \wh{\mu}, \wh{\mu}) > h(w - \alpha \wh{\mu}, \wh{\mu})?
\]
For $w = 0$, this is true by Lemma~\ref{lem:hvCv}.

\subsection{Understanding $w+\alpha v$ vs $w - \alpha v$}
First, let's try and understand $\frac{1}{n \lam} \sum_i \psi(\lam \inner{w+\alpha v, X_i - C v})$ vs $\frac{1}{n \lam}\sum_i \psi(\lam\inner{w-\alpha v, X_i - Cv})$.

\paragraph{Strategy.} Let $a_i = \lam(\inner{w , X_i})$ and $b_i = \lam(\inner{\alpha v, X_i - C v})$. We're looking at something that looks like $\frac{1}{n \lam} \sum_i (\psi(a_i + b_i) -  \psi(a_i - b_i))$ Note that $\frac{1}{n \lam}\sum_i 2 \psi(b_i)$ is *morally* at most $0$ (modulo the expectation over $\theta$ stuff), by the argument in the previous section. So, we would like it if $\psi(a_i+b_i) - \psi(a_i - b_i) \le 2\psi(b_i)$ or some such thing (which is not true, consider $a = \sqrt{2}, b = -\sqrt{2}$. Then, $\psi(a+b) = 0, \psi(a - b) = \frac{2 \sqrt{2}}{3}, \psi(b) = -\frac{2 \sqrt{2}}{3}$).

 $\psi(a+b) - \psi(a) \le \psi(b)$ and $\psi(a-b) - \psi(a) \ge -\psi(b)$ for $b \ge 0$.

 We can assume wlog that $\sum_i \psi(a_i - b_i) \le 0$. (Why? Because if it's $> 0$, we are done since then $\sum_i \psi(-a_i + b_i) \le 0$, which is a direction that is good for us). Given this and $\sum_i \psi(b_i) \le 0$, we want to show that $\sum_i (\psi(a_i +b_i) - \psi(a_i - b_i))\le 0$.

 \begin{align*}
     \sum_{i} \psi(b_i/\alpha) \le 0
 \end{align*}
 It seems like we don't know anything about $\sum_i\psi(b_i)$.

\subsection{Other ideas }
\begin{lemma}
    XXX I don't know what the right version is here, this is true without the random $\theta$ but the expectation makes things annoyingXXX For $v$ orthogonal to $w$, we have
    \[
        h(w, av) \approx h(w, bv)
    \]
\end{lemma}
Even if the above is true, I'm confused about something. What happens for $w$ with some (say positive) projection on $v$? Then it could be that $h(w, Cv) < 0$. But again, we should expect $h(w, av)$ to be monotonically increasing in $a$. So then, it seems like moving closer to the true mean is making the objective worse, which is not good.

Maybe this is resolved by observing the following.
\begin{lemma}
    Suppose $h(v, Cv) \ge 0$ for all $v \in S^{d-1}$.
    Then, for every $w \in S^{d-1}$ and every $\hat \mu$ with $\|\hat \mu\| \ge C$, 
    \[
        h(w, \hat \mu) \ge h\left(w, C \frac{\hat \mu}{\|\hat \mu\|}  \right)
    \]
\end{lemma}
\section{Multivariate Laplace idea}
$Y = \sqrt{Z} X$ where $Z$ is exponential, and $X$ is $N(\mu, 1)$ is Laplace. $Z$ can be replaced with a different distribution to get the Catoni distribution.
\begin{lemma}
    
\end{lemma}
\begin{proof}
    Let $w_{\sigma^2}$ be the density function of $\mathcal N(\mu, \sigma^2)$. Note that $\Pr(Y = y | Z = z) = w_z(y)$. So, we have
    \[
        \Pr(Z=z|Y = y) = \frac{\Pr(Z = z, Y = y)}{\Pr(Y=y)} = \frac{p_Z(z) w_z(y)}{p_Y(y)}
    \] 
    So,
    \begin{align*}
        p_Y(y+\eps) &= \int_{-\infty}^\infty p_Z(z) w_z(y+\eps) dz\\
        &= \int_{-\infty}^\infty \Pr(Z = z | Y = y) p_Y(y) \frac{w_z(y+\eps)}{w_z(y)} dz\\
        &= p_Y(y) \E_{Z | y}\left[ \frac{w_z(y+\eps)}{w_z(y)}\right]\\
        &= p_Y(y) \E_{Z | y}\left[ e^{\frac{-(y+\eps - \mu)^2 + (y - \mu)^2}{2 z}}\right]\\
        &= p_Y(y) \E_{Z | y}\left[e^{\frac{-\eps(y-\mu) + \eps^2}{2z}} \right]
    \end{align*}
\end{proof}
%\input{norm_talagrand.tex}
$Y = \sqrt{Z} X$ where $X \sim \mathcal N(0, I_d)$.
\begin{align*}
    L_Y(y) &= \int \Pr[Z = z] \Pr[Y = y | Z = z] dz
    &= \int \Pr[Z = z] \prod_i \Pr[Y_i = y_i | Z = z] dz
\end{align*}

\begin{align*}
    L_{Y_i}(y) = \int \Pr[Z = z] \Pr[Y_i = y_i | Z = z]dz
\end{align*}

\section{Lower Bound}

\subsection{1-d Gaussian case}
For $f = \mathcal N(0, 1)$, $f^{2\eps} = \mathcal N(2 \eps, 1)$,
\begin{align*}
    &D_{KL}(f || f^{2\eps}) = 2 \eps^2\\
    &d_H^2(f, f^{2\eps}) = 1 - e^{-\frac{\eps^2}{2}} = \frac{\eps^2}{2} + O(\eps^4) \le (1 + O(\eps^2)) \frac{1}{4} D_{KL}(f||f^{2 \eps})\\
    &\E_f\left[|\gamma|^k \right] = \E_f\left[|- 2\eps x + 2\eps^2|^k \right] \le 
\end{align*}

\subsection{Attempt at simplified Hellinger-KL Lemma}
\begin{lemma}
    Suppose we have distributions $p, q$. For a given $x$, let $\gamma = \log \frac{q(x)}{p(x)}$ be the log-likelihood ratio. Suppose also that there is a parameter $\kappa < 0.01$ such that
    \begin{enumerate}
        \item $d_H^2(p, q) \le (1 + \kappa)\frac{1}{4} \min(D_{KL}(p\|q), D_{KL}(q\|p))$
        \item $\E_p\left[|\gamma|^k\right] \le (1 + \kappa) \cdot 2 D_{KL}(p\|q) \cdot \kappa^{k-2}\cdot \frac{k!}{2}$
    \end{enumerate}
\end{lemma}

\begin{proof}
    Note that by condition 1, the Bhattacharya coefficient, $BC(p, q) = \int \sqrt{p(x) q(x)} dx$ has
    \begin{align*}
        BC(p, q) &= 1 - d_H^2(p, q)\\
        &\ge 1 - (1 + \kappa) \frac{1}{4} \min(D_{KL}(p\|q), D_{KL} (q\|p))\\
        &\ge e^{-\frac{1}{4}(1+\kappa) \min(D_{KL}(p\|q), D_{KL}(q\|p)) \cdot (1 + O(\min(D_{KL}(p\|q), D_{KL}(q\|p))))}
    \end{align*}
    On the other hand,
    \begin{align*}
        BC(p, q) = \int \sqrt{p(x) q(x)} dx = \int p(x) e^{\frac{1}{2} \gamma(x)} dx = \E_{x \sim p}\left[e^{\frac{1}{2} \gamma(x)} \right]
    \end{align*}
    So, by the above, by condition 1, we have
    \begin{align*}
    \E_{x \sim p}\left[e^{\frac{\gamma(x)}{2}} \right] \ge e^{-\frac{1}{4} (1 + \kappa) \min(D_{KL}(p\|q), D_{KL}(q\|p)) \cdot (1 + O(\min(D_{KL}(p\|q), D_{KL}(q\|p))))}
    \end{align*}
    Now, by condition 2,
    \begin{align*}
        \E_{x \sim p}\left[e^{\lam \gamma} \right] &\le 1 +\lam \E_p[\gamma] + \sum_{k=2}^\infty \frac{\lam^k}{k!} \E_p\left[|\gamma|^k \right]\\
        &\le 1 - D_{KL}(p\|q) + \sum_{k=2}^\infty \lam^k -
    \end{align*}
    Suppose for the sake of contradiction that $\Pr_{x \sim p^{\otimes n}}\left[\bar \gamma(x) \ge 0 \right] < e^{-\frac{n D_{KL}(p\|q)}{4}}$
    Then, we have
    \begin{align*}
        \E_{x \sim p^{\otimes n}}\left[e^{\frac{\bar \gamma(x)}{2}} \right] = 1 + \frac{1}{2} \E_{x \sim p^{\otimes n}}\left[\bar \gamma(x)\right] + \sum_{k=2}^\infty \frac{1}{2^k k!} \E_{x \sim p^{\otimes n}}\left[(\bar \gamma(x) \right]
    \end{align*}
\end{proof}

\subsection{Coin likelihood ratio}
First, let's try and understand the likelihood ratio of two Poissons with parameters $\lam_1, \lam_2$. Here, I'm thinking of $\lam_1 = C \log \frac{1}{\delta}$ and $\lam_2 = (C + 2\eps) \log \frac{1}{\delta}$ for large $C$. Now, for $x \sim Poi(\lam_1)$, we have
\[
\bar \gamma(x) = \log \frac{p_{\lam_2}(x)}{p_{\lam_1}(x)} = \log \left(\frac{e^{-\lam_2 + \lam_1} \lam_2^x}{\lam_1^x} \right) = x \log \frac{\lam_2}{\lam_1} - \lam_2 + \lam_1
\]

\subsubsection{Preliminary calculation}
We want to understand
\begin{align*}
    \Pr_{x \sim Poi(\lam_1)} \left[\gamma(x) \ge 0 \right] = \Pr_{x \sim Poi(\lam_1)} \left[x \ge \frac{\lam_2 - \lam_1}{\log \frac{\lam_2}{\lam_1}} \right] \approx \Pr_{x \sim Poi(\lam_1)} \left[x = \frac{\lam_2 - \lam_1}{\log \frac{\lam_2}{\lam_1}} \right]
\end{align*}
So the question is, what should we set $\eps$ to be so that the RHS above is $\delta$? We know that by the Taylor approximation of the $\log$ probability (from Lee-Valiant)
\begin{align*}
    \ln\left(\Pr_{x \sim Poi(\lam)}[x = k] \right) \approx \frac{-(k - \lam)^2}{2\lam} + \frac{(k-\lam)^3}{6\lam^2}
\end{align*}
Setting this equal to $\log \delta$ gives that $k = \frac{1}{3} \log \frac{1}{\delta} + \lam \pm \sqrt{2 \lam \log \frac{1}{\delta}}$. So, in our situation, we need
\begin{align*}
    \frac{\lam_2 - \lam_1}{\log \frac{\lam_2}{\lam_1}} = \frac{1}{3} \log \frac{1}{\delta} + \lam_1 + \sqrt{2 \lam_1 \log \frac{1}{\delta}}
\end{align*}
In our case, for $\lam_1 = C \log \frac{1}{\delta}$, $\lam_2 = (C + 2 \eps) \log \frac{1}{\delta}$,
\begin{align*}
    \frac{2 \eps \log \frac{1}{\delta}}{\log \left(1 + \frac{2\eps}{C}\right)} = \frac{1}{3} \log \frac{1}{\delta} + C \log \frac{1}{\delta} + \sqrt{2 C} \log \frac{1}{\delta}
\end{align*}
So numerically, for $C = 10000$, the equation is satisfied for $\eps \approx \sqrt{2 * 10000}$ as expected.
More formally,


\subsubsection{XXX SCRATCH}
Recall that we have by Poisson concentration (aka Bennett's inequality),
\begin{align*}
    \Pr_{x \sim Poi(\lam)} \left[X \ge \lam + t \right] \le e^{-\frac{t^2}{2 \lam} h(\frac{t}{\lam})}
\end{align*}
where $h(u) = 2 \frac{(1 + u)\log (1+u) - u}{u^2}$
So,
\begin{align*}
    \Pr_{x \sim Poi(\lam_1)}\left[\bar \gamma(x) \ge 0 \right] &= \Pr_{x \sim Poi(\lam_1)}\left[x \ge \frac{\lam_2 - \lam_1}{\log \frac{\lam_2}{\lam_1}} \right] = \Pr_{x \sim Poi(\lam_1)}\left[x \ge \lam_1 + \frac{\lam_2 - \lam_1(1 + \log\frac{\lam_2}{\lam_1})}{\log \frac{\lam_2}{\lam_1}} \right]\\
\end{align*}
Now, for $t = \frac{\lam_2 - \lam_1(1 + \log \frac{\lam_2}{\lam_1})}{ \log \frac{\lam_2}{\lam_1}}$, since $1 + \frac{t}{\lam_1} = \frac{\lam_2 - \lam_1}{\log \frac{\lam_2}{\lam_1}}$,
\begin{align*}
    h\left(\frac{t}{\lam_1}\right) = \frac{2 \lam_1^2}{t^2} \cdot\left(\left(\frac{\lam_2 - \lam_1}{\log\frac{\lam_2}{\lam_1}} \right) \log \left(\frac{\lam_2 - \lam_1}{\log \frac{\lam_2}{\lam_1}} \right) - \frac{t}{\lam_1} \right)
\end{align*}

\subsection{1d estimation doesn't work for triangle example}
\text{(Incorrect) Hypothesis:} Estimating each vertex is sufficient to get small error.

Recall that we sample $Poi(\lam+2 \eps)$ on one of the vertices, and $Poi(\lam)$ on the other two vertices. Now, the maximum variance in any direction is $\approx \lam + \frac{1}{4} \lam + \frac{1}{4} \lam = \frac{3}{2} \lam$. This means we need our error to be at most $\sqrt{3 \lam \log \frac{1}{\delta}}$. That is, we need $\sqrt{3} \eps \le \sqrt{3 \lam \log \frac{1}{\delta}}$, or $\eps \le \sqrt{\lam \log \frac{1}{\delta}}$.

But since the $1d$ problem is about trying to distinguish $\lam$ from $\lam + 2 \eps$, and we can only distinguish $\lam$ from $\lam + 2 \sqrt{2 \lam \log \frac{1}{\delta}}$, we cannot do the task. (We need twice as many samples)

\subsection{Using the maximum as an estimator}

On the other hand, using the mean corresponding to the maximum vertex does work. Let's look at $X_1 - X_2$, where $X_1 \sim Poi(\lam + 2 \eps)$ and $X_2 \sim Poi(\lam)$. Since the biases cancel out, the difference is well approximated by a Gaussian. That is $X_1 -X_2 \approx \sim \mathcal N(2 \eps, 2 \lam)$. So, we have that $X_1 - X_2 < 0$ with probability $e^{-\frac{4 \eps^2}{4 \lam}}$. For $\eps = \sqrt{\lam \log \frac{1}{\delta}}$, we do have that $X_1 - X_2 \ge 0$ with probability at least $1 - \delta$.

\subsection{Understanding better}
Suppose I have triangle with $Poi(\lam)$ on each of the vertices. Now let's say I observe the event $\lam + \sqrt{2 \lam \log \frac{1}{\delta}} + \frac{1}{3} \log \frac{1}{\delta}$ on the first vertex and $\lam - \sqrt{2 \lam \log \frac{1}{\delta}} + \frac{1}{3} \log \frac{1}{\delta}$ on the other two vertices. This happens with probability $\approx \delta$.

\section{Duality ish thing}
\subsection{1-d Poisson}
Suppose I see samples either $0$ or $1$, with the number of ones $\sim Poi(\lam)$. Then, if I see $k$ ones for $k = C \log \frac{1}{\delta}$, the distributions that are relevant are ones with parameters $\lam_1 = k - \sqrt{2 k \log \frac{1}{\delta}} - \frac{1}{3} \log \frac{1}{\delta}$ and $\lam_2 = k + \sqrt{2 k \log \frac{1}{\delta}} - \frac{1}{3} \log \frac{1}{\delta}$. To simultaneously satisfy that with probability $1 - \delta$, you are correct for both $Poi(\lam_1)$ and $Poi(\lam_2)$, you *need* to subtract $\frac{1}{3} \log \frac{1}{\delta}$.
\subsection{2d triangle}
Suppose I have samples $k_1, k_2, k_3$ in the triangle case. For a given projection, I need to understand the set of possible distributions that could have generated these samples. Let's restrict ourselves to set of Poissons at each coordinate.

Let's just look in the direction of $k_1$. For any possible $\hat \mu$, we can look at $\lam_1, \lam_2$ such that $\lam_1 - \lam_2 = \hat \mu$ (since there are three Poissons, placed at $1$, $-1/2$, $-1/2$, which is the same as two Poissons at $1, -1/2$). The variance is $\lam_1 + \frac{1}{4} \lam_2$. So, we want that for every $\lam_1, \lam_2$ that could have generated our samples with probability at least $\delta$, $\hat \mu \in [(\lam_1 - \frac{1}{2} \lam_2) - \sqrt{2 (\lam_1 + \frac{1}{4} \lam_2) \log \frac{1}{\delta}}, (\lam_1 - \frac{1}{2} \lam_2) + \sqrt{2 (\lam_1 + \frac{1}{4} \lam_2) \log \frac{1}{\delta}}]$. So, we're looking at
\begin{align*}
    -\frac{(k_1 - \lam_1)^2}{2 \lam_1} + \frac{(k_1 - \lam_1)^3}{6 \lam^2} - \frac{((k_2+k_3) - \lam_2)^2}{2 \lam_2} + \frac{((k_2+k_3) - \lam_2)^3}{6 \lam_2^2} \ge \log \delta
\end{align*}
This is roughly saying 
\begin{align*}
&\lam_1 \in [k_1 - \sqrt{2 k_1 \log \frac{1}{\delta}} - \frac{1}{3} \log \frac{1}{\delta}, k_1 + \sqrt{2 k_1 \log \frac{1}{\delta}} - \frac{1}{3} \log \frac{1}{\delta}]\\
&\lam_2 \in [(k_2+k_3) - \sqrt{2 (k_2 + k_3) \log \frac{1}{\delta}} - \frac{1}{3} \log \frac{1}{\delta}, (k_2+k_3) + \sqrt{2 (k_2 + k_3) \log \frac{1}{\delta}} - \frac{1}{3} \log \frac{1}{\delta}]
\end{align*}
So,

\subsection{Warmup: Gaussians}
Suppose I see $n$ samples, each one equal to $1$ with probability $\mu_1/n$ and $-1$ with probability $\mu_2/n$, and $0$ otherwise. Note that the true mean is $(\mu_1 - \mu_2)/n$ and true variance is $((\mu_1 + \mu_2)/n) (1 + o(1))$. I'll assume $\mu_1, \mu_2 \gg \log \frac{1}{\delta}$ so that we don't have issues of bias. Basically I'm seeing $\mathcal N(\mu_1, \mu_1)$ samples at $1$ and $\mathcal N(\mu_2, \mu_2)$ samples at $-1$. I want to output an interval of estimates. Note that the mean of this distribution is $\mu_1 - \mu_2$, and variance is $\mu_1 + \mu_2$. I see $k_1$ samples on $1$ and $k_2$ samples on $-1$. I want to then distribute probability $\delta_1, \delta_2$ between the Gaussians so that $\delta_1 \cdot \delta_2 = \delta$, and in this case, I want to say that I see $k_1$ with probability $\ge \delta_1$ under $\mu_1$, and $k_2$ with probability $\ge \delta_2$ under $\mu_2$, and I want to find the most extreme such $\mu_1, \mu_2$. Each such $\mu_1, \mu_2$ gives me a constraint on my interval of outputs.

\textbf{Notation:} For sake of simplicity, let $\eps_i = \sqrt{2 k_i \log \frac{1}{\delta}}$.

As an example, if $\delta_1 = \delta_2 = \sqrt{\delta}$, then $\mu_1 = k_1 \pm \frac{\eps_1}{\sqrt{2}}$ and $\mu_2 = k_2 \pm \frac{\eps_2}{\sqrt{2}}$. So, the mean is $k_1 - k_2 - \frac{\eps_1 + \eps_2}{\sqrt{2}} \le \mu_1 - \mu_2 \le k_1 - k_2 + \frac{ \eps_1 + \eps_2}{\sqrt{2}}$, and the variance is $\mu_1 + \mu_2 = k_1 + k_2 + O(\eps_i)$. So any $\hat \mu$ in our output interval must satisfy
\begin{align*}
    (k_1 - k_2) + \frac{\eps_1 + \eps_2}{\sqrt{2}} - \sqrt{2 (k_1 + k_2) \log \frac{1}{\delta}} \le \hat \mu \le (k_1 - k_2) - \frac{\eps_1 + \eps_2}{\sqrt{2}} + \sqrt{2 (k_1 + k_2) \log \frac{1}{\delta}}
\end{align*}

On the other hand, if $\delta_1 \to \delta$ and $\delta_2 \to 1$, then $\mu_1 = k_1 \pm \eps_1$, and $\mu_2 = k_2$. So, the mean is $k_1 - k_2 - \eps_1 \le \mu_1 - \mu_2 \le k_1 - k_2 + \eps_1$ and the variance is again $\mu_1 + \mu_2 = k_1 + k_2 + O(\eps)$. So any $\hat \mu$ in our output interval must satisfy
\begin{align*}
    (k_1 - k_2) + \eps_1 - \sqrt{2 (k_1 + k_2) \log \frac{1}{\delta}} \le \hat \mu \le (k_1 - k_2) - \eps_1 + \sqrt{2(k_1 + k_2) \log \frac{1}{\delta}}
\end{align*}

Note that when $k_1 = k_2 = k$, the first constraint ``dominates'', and you get that the output should be basically just $0$, while if $k_1 = k$ and $k_2 = 0$, the second constraint ``dominates'', and you get that the output should basically be $k$.

In the general case. We'll let $\delta_1 = \delta^x$ and $\delta_2 = \delta^{1-x}$. If you do the calculation, we want to maximize for $0 \le x \le 1$ the following
\begin{align*}
    \eps_1 \sqrt{x} + \eps_2 \sqrt{1 - x} - \sqrt{2(k_1 + k_2) \log \frac{1}{\delta}}
\end{align*}
Setting $x = \frac{k_1}{k_1 + k_2}$ makes this $0$. 
%We can always find an $x$ that makes this $0$.

This means the only time you actually get an interval instead of a point is if $\mu_1, \mu_2 = O(\log \frac{1}{\delta})$.

\section{Poissons}
Same setting as above, except Poissons now (and so $\mu_1, \mu_2 \approx C \log \frac{1}{\delta}$). If $\delta_1 = \delta^x$ and $\delta_2 = \delta^{1-x}$, $\mu_1 = k_1 \pm \eps_1 \sqrt{x} - \frac{x}{3} \log \frac{1}{\delta}$ and $\mu_2 = k_2 \pm \eps_2 \sqrt{1-x} - \frac{1-x}{3} \log \frac{1}{\delta}$. Then, mean is $(k_1 - k_2) - \eps_1 \sqrt{x} - \eps_2 \sqrt{1 - x} + \frac{1-2x}{3} \log \frac{1}{\delta} \le \mu_1 - \mu_2 \le (k_1 - k_2) + \eps_1 \sqrt{x} + \eps_2 \sqrt{1 - x} + \frac{1-2x}{3} \log \frac{1}{\delta} $ and variance is $\mu_1 + \mu_2$. Now if $k_i = C_i \log \frac{1}{\delta}$, for the mean upper bound, the variance is $k_1 + k_2 + \eps_1 \sqrt{x} - \eps_2 \sqrt{1 - x} - \frac{1}{3} \log \frac{1}{\delta} = (C_1 + C_2 + \sqrt{2 C_1 x} - \sqrt{2 C_2 (1 - x)} - \frac{1}{3}) \log \frac{1}{\delta}$ and for the lower bound it's $k_1 + k_2 - \eps_1 \sqrt{x} + \eps_2 \sqrt{1 - x} - \frac{1}{3} \log \frac{1}{\delta} = (C_1 + C_2 - \sqrt{2 C_1 x} + \sqrt{2 C_2 (1 - x)} - \frac{1}{3}) \log \frac{1}{\delta}$

So,
\begin{align*}
    \hat \mu &\le (k_1 - k_2) - \eps_1 \sqrt{x} - \eps_2 \sqrt{1 - x} + \frac{1 - 2x}{3} \log \frac{1}{\delta} +  \sqrt{2(C_1 + C_2 - \sqrt{2 C_1 x} + \sqrt{2 C_2 (1 - x)} - \frac{1}{3}) } \log \frac{1}{\delta}
\end{align*}
For $C_1, C_2$ large, basically $x = \frac{C_1}{C_1 + C_2}$ is going to minimize the RHS. So,
\begin{align*}
    \hat \mu \le (k_1 - k_2) - \sqrt{2 (C_1 + C_2)} \log \frac{1}{\delta} + 
\end{align*}

\subsection{Interesting case}
Poisson at $1$ and $-\frac{1}{2}$. Mean of distribution is $\mu_1 - \frac{1}{2} \mu_2$ and variance is $\approx \mu_1 + \frac{1}{4} \mu_2$.
If $\delta_1 = \delta^x$ and $\delta_2 = \delta^{1-x}$, we have $\mu_1 = k_1 \pm \eps_1\sqrt{x} -\frac{x}{3} \log \frac{1}{\delta}$ and $\mu_2 = k_2 \pm \eps_2 \sqrt{1 - x} - \frac{1-x}{3} \log \frac{1}{\delta}$. So,
\begin{align*}
    (k_1 - \frac{1}{2} k_2) - \eps_1 \sqrt{x} - \frac{\eps_2}{2} \sqrt{1 - x} + \frac{1 - 3x}{6} \log \frac{1}{\delta} \le \mu_1 - \mu_2 \le (k_1 - \frac{1}{2} k_2) + \eps_1 \sqrt{x} + \frac{\eps_2}{2} \sqrt{1 - x} + \frac{1 - 3x}{6} \log \frac{1}{\delta}
\end{align*}
Variance is $k_1 + \frac{1}{4} k_2 + \eps_1 \sqrt{x} - \frac{\eps_2 \sqrt{1 - x}}{4} - \frac{1 - 5x}{12} \log \frac{1}{\delta} = (C_1 + \frac{C_2}{4} + \sqrt{2 C_1 x} - \frac{\sqrt{2 C_2 (1 - x)}}{4} - \frac{1 - 5x}{12}) \log \frac{1}{\delta}$ for the upper bound, which means
\begin{align*}
    \hat \mu \ge (k_1 - \frac{k_2}{2}) + \eps_1 \sqrt{x} + \frac{\eps_2 \sqrt{1 - x}}{2} + \frac{1 - 3x}{6} \log \frac{1}{\delta} - \sqrt{2(C_1 + \frac{C_2}{4} + \cdots)}\log \frac{1}{\delta}
\end{align*}
For $x \approx \frac{k_1}{k_1 + \frac{k_2}{4}}$, this is basically
\begin{align*}
    \hat \mu \ge (k_1 - \frac{k_2}{2}) + \frac{1 - 3x}{6} \log \frac{1}{\delta}
\end{align*}
Similarly, you can get the same upper bound. Note that this is basically just the empirical mean plus $\frac{1 - 3x}{6} \log \frac{1}{\delta}$.

Since by symmetry, the same holds for the other two directions, and you can't put this $\frac{1 - 3x}{6} \log \frac{1}{\delta}$ bias in all three directions simultaneously, there's no two dimensional estimate that is correct for all three projections at once.

\subsection{Full 2-d}
$\delta_1 = \delta^{x_1}, \delta_2 = \delta^{x_2}, \delta_3 = \delta^{x_3}$ for $x_1, x_2, x_3 = 1$. Poissons at $v_1, v_2, v_3$. Mean is $\lam_1 v_1 + \lam_2 v_2 + \lam_3 v_3$, and covariance is $\approx \sum_i \lam_i v_i v_i^T $. Given $k_1, k_2, k_3$ at the three vertices, we have $\lam_i = k_i \pm \eps_i \sqrt{x_i} - \frac{x_i}{3} \log \frac{1}{\delta}$. Let's consider the $+, -, -$ and $-, +, +$ cases. In the $+, -, -$ case, the mean is 
\begin{align*}
    \mu_{+,-,-} &= (k_1 + \eps_1 \sqrt{x_1} - \frac{x_1}{3} \log \frac{1}{\delta}) v_1 + \sum_{i=2, 3} (k_i - \eps_i \sqrt{x_i} - \frac{x_i}{3} \log \frac{1}{\delta}) v_i\\
    &= \left(k_1 - \frac{1}{2}\left(k_2 + k_3 \right) + \eps_1 \sqrt{x_1} + \frac{\eps_2 \sqrt{x_2} + \eps_3 \sqrt{x_3}}{2} + \frac{-2x_1 + x_2 + x_3}{6} \log \frac{1}{\delta} \right) e_1 \\
    &+ \frac{\sqrt{3}}{2} \left((k_3 - k_2) + \eps_2 \sqrt{x_2} - \eps_3\sqrt{x_3} + \frac{x_2 - x_3}{3} \log \frac{1}{\delta}  \right) e_2\\
\end{align*}
and $\|\Sigma_{+,-,-}\|$ is in the $v_1$ direction, given by
\begin{align*}
    &\left(k_1 + \eps_1 \sqrt{x_1} - \frac{x_1}{3} \log \frac{1}{\delta} \right) +\frac{1}{4} \sum_{i=2, 3} \left(k_i - \eps_i \sqrt{x_i} - \frac{x_i}{3} \log \frac{1}{\delta} \right)\\
    &\approx k_1 + \frac{k_2 + k_3}{4}
\end{align*}
So, we have for every $k_1, k_2, k_3$ and every $x_1, x_2, x_3$,
\begin{align*}
    \|\hat \mu - \mu_{+,-,-}\| \le \sqrt{2 \|\Sigma\| \log \frac{1}{\delta}}
\end{align*}
When $k_1 = k_2 = k_3 = k$, and $x_1 = \frac{2}{3}$, $x_2 = x_3 = \frac{1}{6}$,
\begin{align*}
    \mu_{+, -, -} = \left( \sqrt{3 k \log \frac{1}{\delta}} - \frac{1}{6} \log \frac{1}{\delta} \right) v_1
\end{align*}
and
\begin{align*}
    \|\Sigma\| \approx \frac{3}{2} k
\end{align*}
so that
\begin{align*}
    \|\hat \mu - \left( \sqrt{3 k \log \frac{1}{\delta}} - \frac{1}{6} \log \frac{1}{\delta} \right) v_1\| \le \sqrt{3 k \log \frac{1}{\delta}}
\end{align*}
Similarly, you get
\begin{align*}
    \mu_{-,+,+}  = \left(- \sqrt{3k \log \frac{1}{\delta}} - \frac{1}{6} \log \frac{1}{\delta} \right)v_1
\end{align*}
so that
\begin{align*}
     \|\hat \mu - \left(- \sqrt{ 3 k \log \frac{1}{\delta}} - \frac{1}{6} \log \frac{1}{\delta} \right) v_1\| \le \sqrt{3 k \log \frac{1}{\delta}}
\end{align*}
so that $\hat \mu$ must equal $-\frac{1}{6} \log \frac{1}{\delta} v_1$. But, for the $-, +, -$ and $+, -, +$ cases, by symmetry, it must equal $-\frac{1}{6} \log \frac{1}{\delta} v_2$, and for the $-, -, +$ and $+, +, -$ case it must equal $-\frac{1}{6} \log \frac{1}{\delta} v_3$. So, we have the following result
\begin{lemma}[Informal]
    Consider any estimator of the mean that succeeds with probability $1 - \delta$ with confidence radius $r$ for the following distributions (where we place $Poi(\lam_i)$ at $v_i$)
    \begin{itemize}
        \item $\lam_1 = k + \frac{2}{\sqrt{3}}\sqrt{k \log \frac{1}{\delta}} - \frac{2}{9} \log \frac{1}{\delta}, \lam_2 = \lam_3 = k - \frac{1}{\sqrt{3}} \sqrt{k\log \frac{1}{\delta}} - \frac{1}{18} \log \frac{1}{\delta} $
        \item $\lam_1 = k - \frac{2}{\sqrt{3}}\sqrt{k \log \frac{1}{\delta}} - \frac{2}{9} \log \frac{1}{\delta}, \lam_2 = \lam_3 = k + \frac{1}{\sqrt{3}} \sqrt{k\log \frac{1}{\delta}} - \frac{1}{18} \log \frac{1}{\delta} $
        \item $\lam_2 = k + \frac{2}{\sqrt{3}}\sqrt{k \log \frac{1}{\delta}} - \frac{2}{9} \log \frac{1}{\delta}, \lam_1 = \lam_3 = k - \frac{1}{\sqrt{3}} \sqrt{k\log \frac{1}{\delta}} - \frac{1}{18} \log \frac{1}{\delta} $
        \item $\lam_2 = k - \frac{2}{\sqrt{3}}\sqrt{k \log \frac{1}{\delta}} - \frac{2}{9} \log \frac{1}{\delta}, \lam_1 = \lam_3 = k + \frac{1}{\sqrt{3}} \sqrt{k\log \frac{1}{\delta}} - \frac{1}{18} \log \frac{1}{\delta} $
        \item $\lam_3 = k + \frac{2}{\sqrt{3}}\sqrt{k \log \frac{1}{\delta}} - \frac{2}{9} \log \frac{1}{\delta}, \lam_1 = \lam_2= k - \frac{1}{\sqrt{3}} \sqrt{k\log \frac{1}{\delta}} - \frac{1}{18} \log \frac{1}{\delta} $
        \item $\lam_3 = k - \frac{2}{\sqrt{3}}\sqrt{k \log \frac{1}{\delta}} - \frac{2}{9} \log \frac{1}{\delta}, \lam_1 = \lam_2 = k + \frac{1}{\sqrt{3}} \sqrt{k\log \frac{1}{\delta}} - \frac{1}{18} \log \frac{1}{\delta} $
    \end{itemize}
    Then $r \ge \sqrt{2 \|\Sigma\| \log \frac{1}{\delta}} + \frac{1}{6} \log \frac{1}{\delta}$
\end{lemma}
\begin{proof}(Informal)
    Each one generates $k, k, k$ with probability $\delta$, and every point in $\R^2$ is at least $\sqrt{2 \|\Sigma\| \log \frac{1}{\delta}} + \frac{1}{6} \log \frac{1}{\delta}$ away from the mean of one of the $6$ distributions.
\end{proof}
\subsection{Small $C$}
For $k, k, k = C \log \frac{1}{\delta}$, Note that $ x_2 = x_3 = \frac{1 - x_1}{2}$ and $\eps_1 = \eps_2 = \eps_3 = \sqrt{2 k \log \frac{1}{\delta}} = \sqrt{2 C} \log \frac{1}{\delta}$.
\begin{align*}
    \mu_{+, -, -} &= (\eps_1 \sqrt{x_1} + \frac{\eps_2 \sqrt{x_2} + \eps_3 \sqrt{x_3}}{2} + \frac{-2x_1 + x_2 + x_3}{6} \log \frac{1}{\delta}) e_1\\
    &= \left(\eps_1 \left(\sqrt{x_1} + \sqrt{\frac{1 - x_1}{2}}\right) + \frac{1 -3 x_1}{6} \log \frac{1}{\delta}\right) e_1\\
    &= \left(\left(\sqrt{2 C}\left(\sqrt{x_1} + \sqrt{\frac{1 - x_1}{2}}\right) + \frac{1 -3x_1}{6} \right)\log \frac{1}{\delta}\right) e_1
\end{align*}
and
\begin{align*}
    \|\Sigma\| &= \frac{3C \log \frac{1}{\delta}}{2} + \eps_1 \sqrt{x_1} - \frac{\eps_2 \sqrt{x_2} + \eps_3 \sqrt{x_3}}{4}  - \frac{4x_1 + x_2 + x_3}{12} \log \frac{1}{\delta}\\
    &= \frac{3 C \log \frac{1}{\delta}}{2} + \eps_1\left( \frac{2 \sqrt{x_1} - \sqrt{\frac{1 - x_1}{2}}}{2}\right) - \frac{1 + 3x_1}{12} \log \frac{1}{\delta}\\
    &= \left(\frac{3 C}{2} + \sqrt{2 C} \left(\frac{2 \sqrt{x_1} - \sqrt{\frac{1 - x_1}{2}}}{2} \right) - \frac{1 + 3x_1}{12} \right) \log \frac{1}{\delta}
\end{align*}
So, we have
\begin{align*}
    \sqrt{2 \| \Sigma\| \log \frac{1}{\delta}} = \log \frac{1}{\delta} \sqrt{3 C + \sqrt{2 C}\left(2 \sqrt{x} - \sqrt{\frac{1 - x}{2}}\right) - \frac{1 + 3x}{12} }
\end{align*}
So, we basically have
\begin{align*}
    v_1^T\hat \mu &\ge \log \frac{1}{\delta}\left( \sqrt{2 C} \left(\sqrt{x} + \sqrt{\frac{1 - x}{2}}\right) + \frac{1 - 3x}{6}  - \sqrt{3 C + \sqrt{2 C}\left(2 \sqrt{x} - \sqrt{\frac{1 - x}{2}}\right) - \frac{1 + 3x}{12} }\right) \\
    &= \sqrt{3 C} \log \frac{1}{\delta} \left(\sqrt{\frac{2}{3}} \left(\sqrt{x} + \sqrt{\frac{1 - x}{2}} \right) + \frac{1 - 3x}{6 \sqrt{3 C}} - \sqrt{1 + \frac{\sqrt{2}}{3 \sqrt{C}} \left(2 \sqrt{x} - \sqrt{\frac{1 - x}{2}} \right) - \frac{1 + 3x}{36 C}}\right)
    %&= \sqrt{2 C} \log \frac{1}{\delta}\left( \sqrt{x}+ \sqrt{\frac{1 - x}{2}} + \frac{1 - 3x}{6 \sqrt{2 C}} - \sqrt{\frac{3}{2} + \frac{1}{\sqrt{2C}} \left(2 \sqrt{x} - \sqrt{\frac{1 - x}{2}} \right) - \frac{1 + 3x}{24 C}}\right)
\end{align*}

\begin{align*}
    \sqrt{\frac{2}{3}} \left(\sqrt{\frac{2}{3}} + \sqrt{\frac{1 - \frac{2}{3}}{2}} \right) = \sqrt{\frac{2}{3}} \left(\sqrt{\frac{2}{3}} + \sqrt{\frac{1}{6}} \right) = \frac{2}{3} + \frac{1}{3} = 1
\end{align*}

\begin{align*}
    \frac{1 - 3x}{6 \sqrt{3 C}} = \frac{-1}{6 \sqrt{3 C}}
\end{align*}
Similarly, from the $-, +, +$ case, you'll get
\begin{align*}
    v_1^T \hat \mu \le \log \frac{1}{\delta}\left( -\sqrt{2 C} \left(\sqrt{x} + \sqrt{\frac{1 - x}{2}}\right) + \frac{1 - 3x}{6}  + \sqrt{3 C + \sqrt{2 C}\left(2 \sqrt{x} - \sqrt{\frac{1 - x}{2}}\right) - \frac{1 + 3x}{12} }\right)
\end{align*}

\section{Redoing calculations}
\subsection{Simplest case - single Poisson}
Suppose I see $k$. The question is: what $\lambda$ could have generated $k$ with probability at least $\delta$? So, we want to find the $\lam$ such that
\begin{align*}
    - \frac{(k - \lam)^2}{2\lam} + \frac{(k-\lam)^3}{6\lam^2} \ge \log \delta
\end{align*}

\textbf{Claim:} $\lam = k \pm \sqrt{2 k \log \frac{1}{\delta}} + \frac{2}{3} \log \frac{1}{\delta}$ satisfy the equation up to lower order terms.

\textbf{Proof:}
For $\lam = k + \sqrt{2k \log \frac{1}{\delta}} + \frac{2}{3}\log \frac{1}{\delta}$, the LHS is
\begin{align*}
    &\approx -\frac{(-\sqrt{2k \log \frac{1}{\delta}} - \frac{2}{3} \log \frac{1}{\delta})^2}{2(k + \sqrt{2 k \log \frac{1}{\delta}})} + \frac{-2 \sqrt{2} k^{3/2} \log^{3/2} \frac{1}{\delta}}{6 k^2} \approx - \frac{2 k \log \frac{1}{\delta} + \frac{4}{3} \sqrt{k} \log^{3/2} \frac{1}{\delta}}{2(k + \sqrt{2 k \log \frac{1}{\delta}})} - \frac{1}{3} \sqrt{\frac{2}{k}} \log^{3/2} \frac{1}{\delta}\\
    &= - \frac{\log \frac{1}{\delta} + \frac{2}{3} \sqrt{\frac{2}{k}} \log^{3/2}\frac{1}{\delta}}{(1 + \sqrt{\frac{2}{k} \log \frac{1}{\delta}})} - \frac{1}{3} \sqrt{\frac{2}{k}} \log^{3/2} \frac{1}{\delta}\\
    &\approx - \left(\log \frac{1}{\delta} + \frac{2}{3} \sqrt{\frac{2}{k}} \log^{3/2} \frac{1}{\delta} \right)\left(1 - \sqrt{\frac{2}{k} \log \frac{1}{\delta}} \right) - \frac{1}{3} \sqrt{\frac{2}{k}} \log^{3/2} \frac{1}{\delta}\\
    &\approx - \log \frac{1}{\delta} - \frac{2}{3} \sqrt{\frac{2}{k}} \log^{3/2} \frac{1}{\delta} + \sqrt{\frac{2}{k}} \log^{3/2} \frac{1}{\delta} - \frac{1}{3} \sqrt{\frac{2}{k}} \log^{3/2} \frac{1}{\delta}\\
    &= \log \delta
\end{align*}
Similarly for the other $\lam$.

Now the question is, if I see $k$, what should my output $\hat \mu$ be? For every $\lam$ that could have generated $k$ with probability at least $\delta$, it must be that $\hat \mu \in [\lam - \sqrt{2 \lam \log \frac{1}{\delta}}, \lam + \sqrt{2 \lam \log \frac{1}{\delta}}]$. So, since we established that the $\lam$ that can generate $k$ with probability at least $\delta$ are $\lam = k \pm \sqrt{2k \log \frac{1}{\delta}} + \frac{2}{3} \log \frac{1}{\delta}$, we have
\begin{align*}
    \hat \mu &\ge k + \sqrt{2 k \log \frac{1}{\delta}} + \frac{2}{3} \log \frac{1}{\delta} - \sqrt{2 (k + \sqrt{2k \log \frac{1}{\delta}} + \frac{2}{3} \log \frac{1}{\delta}) \log \frac{1}{\delta}}\\
    &\approx k + \sqrt{2k \log \frac{1}{\delta}} + \frac{2}{3} \log \frac{1}{\delta} - \sqrt{2k \log \frac{1}{\delta}} \cdot \sqrt{1 + \sqrt{\frac{2}{k} \log \frac{1}{\delta}}}\\
    &= k + \sqrt{2k \log \frac{1}{\delta}} + \frac{2}{3} \log \frac{1}{\delta} - \sqrt{2k \log \frac{1}{\delta}} - \log \frac{1}{\delta}\\
    &= k - \frac{1}{3} \log \frac{1}{\delta}
\end{align*}
Similarly, (using the other side), you have
\begin{align*}
    \hat \mu \le k - \frac{1}{3} \log \frac{1}{\delta}
\end{align*}
so that subtracting $\frac{1}{3} \log \frac{1}{\delta}$ is the right thing.


\section{More Precise Analysis}

\subsection{Single Poisson}

We want to Taylor expand $\log(\frac{e^{-\lam}\lam^k}{k!})$ for $k$ around $\lam = k$.
 We have, by Stirling's approximation
\begin{align*}
    \frac{e^{-\lam} \lam^{k}}{k!} = e^{-\lam + k} \left(\frac{\lam}{k} \right)^k \frac{1}{\sqrt{2 \pi k}}
 \end{align*}
 Then, letting $t = \lam - k \to 0$, and taking the log,
 \begin{align*}
     \log\left(\frac{e^{-\lam} \lam^{k}}{k!}\right) = -t + k \log \left(1 + \frac{t}{k} \right) - \frac{1}{2} \log (2 \pi k)
 \end{align*}
 Since the last term is $O(\log \log \frac{1}{\delta})$, we can ignore it. Then, the above is
 \begin{align*}
     \log\left(\frac{e^{-\lam} \lam^{k}}{k!}\right) \ge -\frac{t^2}{2k} + \frac{t^3}{3k^2} - \frac{t^4}{4k^3}= -\frac{(\lam - k)^2}{2 k} + \frac{(\lam - k)^3}{3 k^2} - \frac{(\lam - k)^4}{4 k^3}
 \end{align*}
 since the remainder term is positive.

\textbf{Claim: } For $\lam = k \pm \sqrt{2 k \log \frac{1}{\delta}} + \frac{2}{3} \log \frac{1}{\delta} \mp \frac{1}{9} \frac{\log^{3/2}\frac{1}{\delta}}{\sqrt{k}}$, the RHS is at least $\log \delta$.

\textbf{Proof:} Let's consider the case of $\lam = k + \sqrt{2 k \log \frac{1}{\delta}} + \frac{2}{3} \log \frac{1}{\delta}$ first.
\begin{align*}
    -\frac{(\lam - k)^2}{2k} + \frac{(\lam - k)^3}{3 k^2} - \frac{(\lam - k)^4}{4 k^3} &= 
\end{align*}   

 \section{Robust Estimation}

 \subsection{Statistical lower bound?}

    Let $T$ be the triangle with vertices $(0, 0), (\sqrt{3}\alpha/2, \alpha/2), (-\sqrt{3} \alpha/2, \alpha/2)$.
 Want to compute 

 \begin{align*}
     \frac{1}{3} - \text{Vol($\mathcal N(0, I), T$)} + \text{Vol($\mathcal N((0, \alpha), I), T$)}
 \end{align*}
    We have
 \begin{align*}
     \text{Vol($\mathcal N((0, \alpha), I), T$)} = \int_{-\sqrt{3}\alpha}^{\sqrt{3} \alpha} \int_{0}^{\alpha(1 - x/\sqrt{3})} w_{(0, \alpha)}(x, y) dy dx
 \end{align*}
 and
 \begin{align*}
     \text{Vol($\mathcal N(0, I), T$)} = \int_{-\sqrt{3}\alpha}^{\sqrt{3} \alpha} \int_{0}^\alpha w_{0}(x, y) dy dx - \int_{-\sqrt{3} \alpha}^{\sqrt{3}\alpha}  
 \end{align*}

 \section{Computational Lower bound - Robust covariance estimation}
 Distinguishing between
 \begin{itemize}
     \item $D_0 = \mathcal N(0, 1)^{\otimes n d}$
     \item $D_1:$ First sample random unit vector $v \in \R^d$. Then, draw $n$ vectors $X_1, \dots, X_n$ from
     \[
        P_v(x) = A(v \cdot x) \exp(- \|x - (v \cdot x) v\|^2 /2)/(2 \pi)^{(n-1)/2}
     \]
     where $A = (1 - \eps) \mathcal N(0, (1/5 - \eps)/(1 - \eps)) + (\eps/2) \mathcal N(\sqrt{4/(5 \eps)}, 1) + \eps/2 \cdot \N(-\sqrt{4/(5 \eps)}, 1)$
 \end{itemize}
 \section{Computational lower bound - Heavy tailed covariance estimation} Let's let $Y_1, \dots, Y_n$ be Bernoulli random variables with parameter $p = \frac{n}{d \sqrt{\log \frac{1}{\delta}}} \ll 1$. Let $\eps = \frac{1}{\sqrt{d}} \log^{1/4} \frac{1}{\delta}$ Consider the problem of distinguishing between
 \begin{itemize}
     \item $D_0$: $\N(0, 1)^{\otimes nd}$
     \item $D_1:$ First sample random unit vector $v \in \R^d$, along with $Y_1, \dots, Y_n \sim \text{Bern($p$)}$. Now, if $Y_i = 0$ let $a_i \sim \N(0, (1/5 - \eps)/(1 - \eps))$, and otherwise, let $a_i \sim \frac{1}{2} \N(\sqrt{4/(5 \eps)}, 1) + \frac{1}{2} \N(-\sqrt{4/(5\eps)}, 1)$. Finally, sample $X_i \sim \N(0, I - v v^T) + a_i v$.
 \end{itemize}

 \textbf{Ignore above! Here's a different distinguishing problem:} 
 \textbf{Observation 1:} With probability at least $\delta$, $\eps$ fraction of the $Y_is$ are equal to $1$.

 We condition on the above event.

 First, let's consider a multilinear Hermite polynomials indexed by $\alpha \subseteq [n] \times [d]$. We have

\begin{align*}
 \E_{a, v, Y, X} \left[ H_\alpha(X) \right] = \E_{a, v, Y, X}\left[\prod_{(i, j) \in \alpha} X_{i, j} \right] = \E_{a, v, Y}\left[ \prod_{i} \E_X\left[\prod_{j : (i, j) \in \alpha} X_{i, j} \Big|a, v, Y\right] \right]
 \end{align*}

 Now, let $S_i = \{j : (i, j) \in \alpha\}$. We have
 \begin{align*}
     \E_X\left[\prod_{j : (i, j) \in \alpha} X_{i, j} \Big | a, v, Y\right] &= \E_g\left[\prod_{j \in S_i} (g_{i, j} + a_i v_j) \Big | a, v, Y \right]\\
     &= \E_g\left[\sum_{T \subseteq S_i} g_i^T v^{S_i \setminus T} a_i^{|S_i \setminus T|} \Big | a, v, Y \right]\\
 &= v^{S_i} \sum_{T \subseteq S_i, |T| \text{ even}} (|T| - 1)!! (-1)^{|T|/2} a_i^{|S \setminus T|} \quad \text{by Wick's theorem}
 \end{align*}

\textbf{Sam's idea}
Set $p = \eps - \alpha$, and $\eps$ constant. The variance of $A$ is like $1/5 + (4/5) p/\eps = 1 - O(\alpha)$. The problem is, the gap between the variance of $A$ and $1$ is now just $O(\alpha)$. But we need that the conditional variance is $1$, so that 
\[
    \sqrt{\frac{\eps \log \frac{1}{\delta}}{n}} \approx \alpha
\]
or
\[
    \alpha = O\left(\sqrt{\frac{\log \frac{1}{\delta}}{n}}\right)
\]
(since $\eps$ is a constant)
But the fourth moment in most directions is still $1$. So you must assume that your polynomial time algorithm has error  $\alpha = \sqrt{\frac{\log \frac{1}{\delta}}{n}}$, which is possible even information theoretically.

\section{Statistical Lower bound attempt for robust estimation}

\subsection{1-d}
Consider the case of estimating the mean of an identity covariance distribution robustly. In 1d, the worst case is given by the distributions: $2 \eps$ mass on $-\frac{1}{\sqrt{2\eps}}$ and $1-2\eps$ on $0$ vs $2\eps$ mass on $\frac{1}{\sqrt{2 \eps}}$ and remaining on $0$. Both distributions have variance $1 + O(\eps)$. Both these distributions are $\eps$-close in TV to the distribution placing $\eps$ on $\pm\frac{1}{\sqrt{2 \eps}}$, remaining on $0$. So, any algorithm must incur error at least $\sqrt{2 \eps}$.

\subsection{2d}
Let $v_1, v_2, v_3$ be the vertices of the equilateral triangle. Consider the distributions placing $3\eps/2$ at $\sqrt{\frac{2}{3 \eps}}v_i$  and remaining mass at $0$. The variance in the $v_i$ direction is $1$, while the mean is $\sqrt{\frac{3 \eps}{2}}$ (This is not as good as what we got for the 1d case). Each of these can be corrupted into $\eps/2$ at each of $\sqrt{\frac{2}{3\eps}} v_i$.

You could try putting mass in some different way so that the covariance is $1$ but can be $\eps$ corrupted into the triangle. However, it seems like any of these give the same answer.
For instance, let's try $\frac{3 \eps}{4}$ at $\sqrt{\frac{4}{3 \eps}} e_1$ and $\frac{3 \eps}{4}$ at $\sqrt{\frac{4}{3 \eps}} e_2$. 

\section{Upper bound??}

\textbf{Key observations:}
\begin{itemize}
    \item $TV(v^T X, v^T Y) \le TV(X, Y)$ aka $TV(X, Y) = \eps \implies TV(v^T X, v^T Y) \le \eps$.
    \begin{proof}
        Let $p, q$ be the pdfs of $X, Y$ and let $\Tilde p, \Tilde q$ be the pdfs of $v^T X, v^T Y$. Consider any one dimensional slice. $p, q$ are allowed to drop parts of the slice where $q > p$, while $\Tilde p, \Tilde q$ are not. So the sup must be larger for $p, q$.
    \end{proof}
    \item $Cov(X) \le I \implies Var(v^T X) \le 1$
\end{itemize}

The above are saying that any distribution that *could have* been $\eps$-corrupted into the input distribution "shows up" in 1-d projections. 

So now the situation is the following: We have a bunch of means of the "uncorrupted distributions" $\mu_1, \dots, \mu_k$. We get to see, for every $v$, $v^T \mu_1, \dots, v^T \mu_k$. We then output, for each $v$, an interval of points $[l_v, u_v]$ such that every point in the interval is no more than $R$ away from $\mu_1, \dots, \mu_k$. We are also guaranteed (by the 1d error bound) that the interval is non-empty for $R = \sqrt{2 \eps}$.

\textbf{Claim:} There exists a point $\hat \mu$ such that $v^T \hat \mu \in [l_v, r_v]$ for all $v$.

\begin{proof} sketch: Consider say direction $v = \frac{1}{\sqrt{2}} e_1 + \frac{1}{\sqrt{2}} e_2$. By definition, there exists some point $x \in [l_{e_1}, u_{e_2}]$ and point $y \in [l_{e_2}, u_{e_2}]$ such that both $x, y$ are $R$ close in their respective projections.

The claim is that $\frac{1}{\sqrt{2}} x + \frac{1}{\sqrt{2}} y$ belongs to the interval for $v$. This is because, for any $\mu_i$, by definition of $x, y$,

\[
    |x - e_1^T \mu_i| \le R
\]
and
\[
    |y - e_2^T \mu_i| \le R
\]
So, we have
\begin{align*}
    \left|\frac{1}{\sqrt{2}}\left( x + y \right) - \frac{1}{\sqrt{2}} (e_1 + e_2)^T \mu_i \right| \le 
\end{align*}

\end{proof}

\section{1-d Upper bound -- robust estimation}

Suppose we have distributions $X, Y$ that are both $\eps$-close to $D$. Then,
\begin{align*}
    TV(X, Y) \le 2 \eps
\end{align*}
Now, let's consider the difference in means
\begin{align*}
    \E[X - Y] &= \E[\1_{X \neq Y} (X - Y)]\\
    &\le \sqrt{\E[\1_{X \neq Y}]\E[(X - Y)^2]}\\
    &\le \sqrt{E[(X - Y)^2]} \sqrt{2 \eps}\\
    &\le 2 \sqrt{2 \eps}
\end{align*}
So, the error is at most $\sqrt{2 \eps}$

\section{Lower bound}

\subsection{Robust}
In 2-d, the corrupted distribution is - put $\eps$ at three vertices of the triangle. The clean distributions are, flip one of the vertices across the origin (to get $3$ clean distributions). Then, the algorithm must output $0$. But the mean of the clean distribution is $2\eps$ away from $0$. Also, the covariance is $\frac{3 \eps}{2}$ in each direction. This means we get $C = \frac{8}{3}$ for error $\sqrt{2 C \|\Sigma\|}$, which matches the Jung's theorem bound.


\section{Heavy-Tail upper bound approach}
So far, we have looked at union bounding over many directions. What if we instead try to look at the sum of $k^{th}$ power of the estimates over many directions? We should expect that the $1/k$-power of this sum converges to the max as $k\to \infty$. Can we try and analyze this quantity for the Catoni estimator?

First, for a standard Gaussian, let's let $S$ be a net over the circle. Just to understand, let's let it be the $8$ directions corresponding to an octagon. Then, we have
\begin{align*}
    \sum_{v \in S} (v^T X)^k
\end{align*}

\section{Scratch}
One observation is that it matters which 1-d heavy-tailed estimator you use. Consider the narrow Catoni estimator which has $\psi(x) = \log 2$ for $|x| \ge 1$. We have that for samples placed far enough away at $e_1$, the contribution to $r(\theta_{MoM})$ is $\frac{\log(2) \cdot \sigma}{\sqrt{2 \log \frac{1}{\delta} \cdot n}}$. So for $\frac{2}{\log 2} \log \frac{1}{\delta}$ samples placed far away, the estimated mean is $\sigma \cdot \sqrt{\frac{2 \log \frac{1}{\delta}}{n}}$. But this is true in every direction with some projection onto $e_1$ for samples placed far away enough (in particular, the ones 30 degrees away in both directions).

However, the Lee-Valiant estimator doesn't suffer from this issue.

\section{New idea}

\subsection{Modified Catoni Estimator for coins}
Instead of the family of $\psi$ as in the standard Catoni analysis, we choose a particular $\psi$ as follows (for $c$ slightly smaller than $1$.
\begin{align*}
     \psi(x) = 
        \begin{cases}
            \log(1+x + \frac{cx^2}{2}), \quad x \ge 0\\
            -\log(1 - x + \frac{cx^2}{2}), \quad x < 0
        \end{cases}
\end{align*}
Now suppose our distribution is Bernoulli with parameter $p = \frac{C\log \frac{1}{\delta}}{n}$ for small $C$. Then, out of $n$ samples, with probability $1 - \delta$, we will see $pn \pm \sqrt{2 pn \log \frac{1}{\delta}} + \frac{1}{3} \log \frac{1}{\delta} = (C + \sqrt{2 C} + \frac{1}{3}) \log \frac{1}{\delta}$ ones. Let $T = \sigma \sqrt{\frac{n}{2\log \frac{1}{\delta}}}$ and recall that our estimate in this case is given by (since $0$ is within $O\left(\sigma \sqrt{\frac{\log \frac{1}{\delta}}{n}}\right) = O\left( \frac{\log \frac{1}{\delta}}{n}\right)$ of true mean $p = \frac{C \log \frac{1}{\delta}}{n}$)
\begin{align*}
    r(0) = \frac{T}{n} \sum_{i=1}^n \psi\left(\frac{x_i}{T} \right)
\end{align*}

For $x_i = 1$, 
\begin{align*}
    \frac{T}{n} \psi\left(\frac{x_i}{T} \right) &= \frac{T}{n} \log \left(1 + \frac{1}{T} + \frac{c }{2 T^2}  \right)\\
    &\approx \frac{1}{n} \left(1 - \frac{1 - c}{2T} + \frac{2 - 3c}{6 T^2} \right)
\end{align*}
Since $T = \sigma \sqrt{\frac{n}{2\log \frac{1}{\delta}}} = \sqrt{C/2}$, this is
\begin{align*}
    \frac{1}{n} \left(1 - \frac{1 - c}{\sqrt{2C}} + \frac{2 - 3c}{3 C}\right)
\end{align*}

So, with probability $1 - \delta$
\begin{align*}
    r(0) &\le \frac{\log \frac{1}{\delta}}{n} \left(C + \sqrt{2 C} + \frac{1}{3} \right) \left(1 - \frac{1 - c}{\sqrt{2 C}} + \frac{2 - 3c}{3C} \right)\\
    &\approx \frac{\log \frac{1}{\delta}}{n} \left(C + \sqrt{C} \left(\sqrt{2} - \frac{1 - c}{\sqrt{2}} \right) \right)\\
    &= p + \sqrt{p \log \frac{1}{\delta}} \left(\sqrt{2} - \frac{1 - c}{\sqrt{2}}\right)
\end{align*}
XXX What about the $1/C$ terms above? Seems like these terms are negative, but the expression can't actually be less than $0$, so is fine. So the approximations should actually just be upper bounds.

\subsection{Generic analysis when $x \ge \beta T$ always}
\textbf{Intuition:} Instead of a single coin, we have a varianble that takes values $y_1, \dots y_k$ with probability $p_1, \dots, p_k$, where all $p_j < C \frac{\log \frac{1}{\delta}}{n}$, and $\sum_j p_j y_j^2 = \sigma^2$.

\begin{align*}
    r(\theta_{MoM}) = 
\end{align*}
\subsection{General analysis}
\begin{lemma}
    Let $T = \sigma \sqrt{\frac{n}{\log \frac{1}{\delta}}}$. Let $\beta$ be a small enough constant. For the true mean $\theta$, suppose
    \begin{align*}
        \E\left[(X - \theta)^2 1_{|X - \theta| \ge \beta T} \right] \ge \gamma \sigma^2
    \end{align*}
    Then, for $c < 1$, for
    \begin{align*}
        \psi(x) = 
        \begin{cases}
            \log(1+x + \frac{cx^2}{2}), \quad x \ge 0\\
            -\log(1 - x + \frac{cx^2}{2}), \quad x < 0
        \end{cases}
    \end{align*}
    and 
    \begin{align*}
        r(\theta_{MoM}) = \frac{T}{n} \sum_{i=1}^n \psi\left(\frac{X_i - \theta_{MoM}}{T}\right)
    \end{align*}
    we have, with probability $1 - \delta$
    \begin{align*}
        |(\theta_{MoM} + r(\theta_{MoM}) - \theta| \le (1 - XXX)\sigma\cdot \sqrt{\frac{2 \log \frac{1}{\delta}}{n}}
    \end{align*}
\end{lemma}

\section{Narrow Catoni}

Consider the narrow Catoni $\psi$ function:
\begin{align*}
    \psi(x) = \begin{cases}
        \log(2), \quad &x \ge 1\\
        \log(1 + x + x^2/2), \quad &0\le x < 1\\
        -\log(1 - x + x^2/2), \quad &-1 \le x < 0\\
        - \log(2), \quad &x < -1\\
    \end{cases}
\end{align*}
Also consider the function
\begin{align*}
    r(\theta_{MoM}) = \frac{T}{n} \sum_{i=1}^n \psi\left(\frac{x_i}{T} \right)
\end{align*}
for $T = \sigma \sqrt{\frac{n}{2 \log \frac{1}{\delta}}}$.

Now suppose we have distribution that is $C T$ with probability $p_1$, $-C T$ with probability $p_2$, and $0$ otherwise. This is a generalization of a coin. Note that $\sigma^2 = (p_1 + p_2) (C T)^2 = (p_1 + p_2) (C^2 \sigma^2 \frac{n}{2\log \frac{1}{\delta}})$, so that $p_1 + p_2 = \frac{2 \log \frac{1}{\delta}}{C^2n}$. Note also that the mean is $(p_1 - p_2) CT \le \frac{2 \log \frac{1}{\delta}}{C n} T \le \frac{2 \log \frac{1}{\delta}}{C^2 n}$. With probability $1 - \delta$, we see $p_1 n \pm \sqrt{2 p_1 n \log \frac{1}{\delta}} + \frac{1}{3} \log\frac{1}{\delta}$ samples equal to $1$ and $p_2 n \pm \sqrt{2 p_2 n\log \frac{1}{\delta} } + \frac{1}{3} \log \frac{1}{\delta}$ samples equal to $-1$. We have the following claim.

\begin{lemma}
    With probability $1 - \delta$,
    \begin{align*}
        |r(0)| \le 
    \end{align*}
\end{lemma}
\begin{proof}
    We have
    \begin{align*}
        r(0) = 
    \end{align*}
\end{proof}

\section{Modified Catoni (retry)}

Consider the following Catoni $\psi$ function:

\begin{align*}
    \psi(x) = 
    \begin{cases}
        \log(1 + x + (1 - \eta) x^2/2), \quad &x \ge 1\\
        \log(1 + x + x^2/2), \quad &0 \le x < 1\\
        -\log(1 - x + x^2/2), \quad &-1 \le x < 0\\
        -\log(1 - x + (1 - \eta) x^2/2), \quad &x < -1\\
    \end{cases}
\end{align*}

Consider the associated function, for $T = \sigma \sqrt{\frac{n}{2 \log \frac{1}{\delta}}}$ given by
\begin{align*}
r(\theta_{MoM}) = \frac{T}{n} \sum_{1=1}^n \psi\left(\frac{x_i - \theta_{MoM}}{T} \right) 
\end{align*}
Let's first consider the situation where $\theta_{MoM} = 0$ and $x_i$ takes on only two values: $0$ with probability $1 - p$ and $\frac{T}{1 - \eta}$ with probability $p$. Then, the mean $\theta = p \frac{T}{1 - \eta}$. The variance $\sigma^2 = \frac{T^2}{(1 - \eta)^2} \cdot p$. This means since
\begin{align*}
    T = \sigma \sqrt{\frac{n}{2 \log \frac{1}{\delta}}}
\end{align*}
we have
\begin{align*}
        p = \frac{(1 - \eta)^2 \cdot 2 \log \frac{1}{\delta}}{n}
\end{align*}

Now, we have
\begin{align*}
    \E\left[\exp\left(\frac{n}{T} r(\theta_{MoM})\right) \right] &\le \prod_{i=1}^n \E\left[1 + \frac{x_i}{T} + (1 -\eta) \frac{x_i^2}{2T^2} \right]\\
    &= \prod_{i=1}^n \left(1 + \frac{\theta}{T} + (1 - \eta) \frac{\sigma^2}{2 T^2}\right)\\
    &\le \exp\left(\frac{n\theta}{T} + (1 - \eta) \frac{n \sigma^2}{2T^2} \right) \quad \text{XXX this is an approximation}
\end{align*}
So, by Chernoff bound
\begin{align*}
    \Pr\left[r(0) \ge \theta + \left(1 - \frac{\eta}{2}\right) \cdot \sigma \sqrt{\frac{2 \log \frac{1}{\delta}}{n}} \right] &\le \exp\left((1-\eta)\frac{n \sigma^2}{2 T^2} - \frac{n}{T} \cdot \left(1 - \frac{\eta}{2}\right) \sigma \sqrt{\frac{2 \log \frac{1}{\delta}}{n}} \right)\\
    &= \exp\left((1 - \eta) \log \frac{1}{\delta} - \left(1 - \frac{\eta}{2} \right) \cdot 2 \log \frac{1}{\delta} \right)\\
    &= \delta
\end{align*}

==> heavy_tailed_lower_bound.tex <==
\section{Heavy-Tailed Lower Bound}

%\begin{lemma}
%    For $\lam = C \log \frac{1}{\delta}$ and $x \sim Poi(\lam)$, with probability at least $\delta$,
%    $x = \lam + \sqrt{2 \lam \log \frac{1}{\delta}} + \frac{1}{3} \log \frac{1}{\delta}$ and similarly, with probability at least $\delta$, $x = \lam - \sqrt{2 \lam \log \frac{1}{\delta}} + \frac{1}{3} \log \frac{1}{\delta}$.
%\end{lemma}
%\begin{proof}
%    
%\end{proof}
\begin{lemma}
    \label{lem:precise_poisson_approx}
    Let $k = C \log \frac{1}{\delta}$ for large enough constant $C > 1$. For 
    \[x \sim Poi\left(k + \sqrt{2 k \log \frac{1}{\delta}} + \left(\frac{2}{3} - O\left(\frac{1}{C} \right)\right) \log \frac{1}{\delta} \right)\] with probability at least $\delta$, $x = k$.

    Similarly, for $x \sim Poi\left(k - \sqrt{2 k \log \frac{1}{\delta}} + \left(\frac{2}{3}  + O\left(\frac{1}{C} \right)\right) \log \frac{1}{\delta} \right)$, with probability at least $\delta$, $x = k$.
\end{lemma}

\begin{proof}
Note that $p_k := \Pr[Poi(\lam) = k] = \frac{\lam^k e^{-\lam}}{k!}$. So, by Stirling's approximation, 
\begin{align*}
    \log p_k = - \frac{(k-\lam)^2}{2 \lam} + \frac{(k - \lam)^3 }{6 \lam^2} + \dots
\end{align*}
So, for $\lam = k + \sqrt{2 k \log \frac{1}{\delta}} + \left(\frac{2}{3} - O\left(\frac{1}{C}\right)\right) \log \frac{1}{\delta} $, where $k = C \log \frac{1}{\delta}$, we have
\begin{align*}
        \log p_k &\ge -\frac{\left(-\sqrt{2 k \log \frac{1}{\delta}} - \left(\frac{2}{3} - O(1/C) \right) \log \frac{1}{\delta}\right)^2}{2(k + \sqrt{2 k \log \frac{1}{\delta}} + \left(\frac{2}{3} - O(1/C) \right)\log \frac{1}{\delta})} + \frac{\left(-\sqrt{2 k \log \frac{1}{\delta}} - \left(\frac{2}{3} - O(1/C) \right) \log \frac{1}{\delta}\right)^3}{6 (k + \sqrt{2 k \log \frac{1}{\delta}} + \left(\frac{2}{3} - O(1/C) \right)\log \frac{1}{\delta})^2} - O\left(\frac{1}{C} \right) \log \frac{1}{\delta}\\
        &\ge -\frac{(-\sqrt{2 k \log \frac{1}{\delta}} - \frac{2}{3} \log \frac{1}{\delta})^2}{2 (k + \sqrt{2 k \log \frac{1}{\delta}})} + \frac{-(2k \log \frac{1}{\delta})^{3/2}}{6 k^2} + O\left(\frac{1}{C} \right)\log \frac{1}{\delta}\\
        &\ge - \frac{2 k \log \frac{1}{\delta} + \frac{4}{3} \sqrt{k} \log^{3/2} \frac{1}{\delta}}{2(k + \sqrt{2 k \log \frac{1}{\delta}})} - \frac{1}{3} \sqrt{\frac{2}{k}} \log^{3/2} \frac{1}{\delta} + O\left(\frac{1}{C} \right) \log \frac{1}{\delta}\\
        &\ge - \left(\log \frac{1}{\delta} + \frac{2}{3} \sqrt{\frac{2}{k}} \log^{3/2} \frac{1}{\delta}\right) \left(1 - \sqrt{\frac{2}{k} \log \frac{1}{\delta}} \right) - \frac{1}{3} \sqrt{\frac{2}{k}} \log^{3/2} \frac{1}{\delta} + O\left( \frac{1}{C}\right) \log \frac{1}{\delta}\\
        &\ge \log \delta
\end{align*}
So $x = k$ with probability at least $\delta$.
The other case is similar.
\end{proof}

\begin{lemma}
    \label{lem:abstract_triangle_poisson_approx}
    Let $C$ be a large enough constant, and let $k = C \log \frac{1}{\delta}$. Let $n > O_C\left( \log \frac{1}{\delta}\right)$. Consider a random variable $x$ such that for constant $\alpha \in [0, 1]$
    \begin{itemize}
        \item $x = 1$ with probability $\frac{k - \sqrt{2 \alpha k \log \frac{1}{\delta}} + \alpha \left(\frac{2}{3} + O\left(\frac{1}{C} \right)\right) \log \frac{1}{\delta}}{n}$
        \item $x = 2$ or $x = 3$ with probability $\frac{k + \sqrt{(1 - \alpha) k \log \frac{1}{\delta}} + \left(\frac{1 - \alpha}{3} - O\left(\frac{1}{C} \right) \right)\log \frac{1}{\delta}}{n}$ each
        \item $x = 0$ otherwise
    \end{itemize}
    Then, given $n$ samples $x_1, \dots, x_n$ with probability at least $\delta$, $\sum_{i=1}^n \1_{\{x_i = j\}} = k$ for each $j \in \{1, 2, 3\}$.
\end{lemma}
\begin{proof}
    We make use of the Poisson approximation. Let $p_j = \Pr[x_i = j]$ and let $y_j \sim Poi(n p_j)$ be independent random variables for each $j \in \{0, \dots, 3\}$. Let $E$ be the event that $\sum_{i=1}^n \1_{\{x_i = j\}}$ for each $j \in \{1, 2, 3\}$. We know that
    \begin{align*}
        \Pr\left[E \right] = \Pr\left[(y_1, y_2, y_3, y_4) = (n-3k, k, k, k) \Big | \sum_{j=1}^4 y_j = n  \right] \ge \Theta(\sqrt{n}) \cdot \Pr\left[ (y_1, y_2, y_3, y_4) = (n-3k, k, k, k) \right]
    \end{align*}
    since $\Pr[Poi(n) = n] = \Theta\left(\frac{1}{\sqrt{n}} \right)$ by Stirling's approximation. Similarly, $\Pr[y_1 = n - 3 k] = \Theta\left(\frac{1}{\sqrt{n}}\right)$ for our choice of $k = C \log \frac{1}{\delta}$ since $n > O_C(\log \frac{1}{\delta})$. Then, putting this together with Lemma~\ref{lem:precise_poisson_approx}, we have
    \begin{align*}
        \Pr\left[(y_1, y_2, y_3, y_4) = (n - 3k, k, k, k) \right] \ge \Theta\left(\frac{1}{\sqrt{n}} \cdot \delta^{\alpha} \cdot \delta^{\frac{1 - \alpha}{2}} \cdot \delta^{\frac{1 - \alpha}{2}} \right) \ge \Theta\left(\frac{\delta}{\sqrt{n}} \right)
    \end{align*}
    So, 
    \begin{align*}
        \Pr[E] \ge O(\delta)
    \end{align*}
    Reparameterizing $\delta$ and noting that $n > O_C(\log \frac{1}{\delta})$ gives the claim. 
\end{proof}

\heavylowerthm*
%\begin{theorem}
%    Let $C$ be a large enough constant and let $n > O_C(\log \frac{1}{\delta})$. There exists a set of two-dimensional distributions with covariance $\Sigma \preccurlyeq \sigma^2 I_2$ such that, given $n$ samples, with probability at least $\delta$, it is impossible to distinguish between them, but the circumradius $R$ of their means has
%    \begin{align*}
%        R \ge (1 + \tau) \cdot \sigma \sqrt{\frac{2 \log \frac{1}{\delta}}{n}}
%    \end{align*}
%    for some constant $\tau > 0$.
%\end{theorem}
\begin{proof}
    Let $v_1, v_2, v_3$ be the vertices of a regular triangle centered at the origin, with $\|v_i\| = 1$. Fix $k = C \log \frac{1}{\delta}$. Fix $\alpha = 2/3$. For each $j \in [3]$, let $D_j$ be the $2$-dimensional distribution that is 
    \begin{itemize}
        \item
        $v_j$ with probability $\frac{k - \sqrt{2 \alpha k \log \frac{1}{\delta}} + \alpha \left(\frac{2}{3} +O\left(\frac{1}{C} \right)\right) \log \frac{1}{\delta}}{n}$
        \item $v_i$ for $i \neq j$ with probability $\frac{k + \sqrt{(1 - \alpha) k \log \frac{1}{\delta}} + \left(\frac{1 - \alpha}{3} - O\left(\frac{1}{C} \right) \right)\log \frac{1}{\delta}}{n}$ each
        \item $0$ otherwise
    \end{itemize}
    By Lemma~\ref{lem:abstract_triangle_poisson_approx}, for $n$ samples distributed according to $D_j$, with probability at least $\delta$, $k$ samples will be placed on each of $v_1, v_2, v_3$, for each $D_j$. Thus, with probability at least $\delta$, any mean-estimation algorithm must incur error lower bounded by the radius of the minimum enclosing ball of the means of the $D_j$s.
    
    For $\alpha = 2/3$, the mean of $D_j$ is given by
    \begin{align*}
        \mu_j &= \frac{\log \frac{1}{\delta}}{n} \left(- \sqrt{2 \alpha C} + \alpha \left(\frac{2}{3} + O\left(\frac{1}{C} \right) \right) - \sqrt{(1 - \alpha) C} + \left(\frac{1 - \alpha}{3} + O\left(\frac{1}{C} \right)\right) \right) v_j\\
        &= \frac{\log \frac{1}{\delta}}{n} \left(- \sqrt{3 C} + \frac{1}{3} + O\left(\frac{1}{C} \right)\right) v_j
    \end{align*}
    The covariance of $D_j$ is given by
    \begin{align*}
        \Sigma_j = \frac{\log \frac{1}{\delta}}{n} \left(\left(C - \sqrt{2 \alpha C} + \frac{2 \alpha}{3} + O\left(\frac{1}{C} \right)  \right)v_j v_j^T + \sum_{i \neq j}\left(C +\sqrt{(1 - \alpha) C} + \frac{1 - \alpha}{3} - O\left(\frac{1}{C} \right)\right)v_i v_i^T \right)
    \end{align*}
    For $\alpha = 2/3$,
    \begin{align*}
        v_j^T \Sigma_j v_j = \frac{\log \frac{1}{\delta}}{n} \left( \frac{3C}{2} - \frac{\sqrt{3 C}}{2} + \frac{1}{2} + O\left( \frac{1}{C}\right)\right)
    \end{align*}
    So, we have
    \begin{align*}
        \sqrt{v_j^T \Sigma_j v_j \cdot \frac{2 \log \frac{1}{\delta}}{n}} = \frac{\log \frac{1}{\delta}}{n} \left(\sqrt{3 C} - \frac{1}{2} + O\left(\frac{1}{\sqrt{C}} \right) \right)
    \end{align*}
    So, for $\alpha=2/3$,
    \begin{align*}
        \sigma^2 = \|\Sigma_j\| = v_j^T \Sigma_j v = \frac{\log \frac{1}{\delta}}{n} \left(\frac{3 C}{2} - \frac{\sqrt{3 C}}{2} + \frac{1}{2} + O\left( \frac{1}{C}\right) \right) 
    \end{align*}
    Then,
    \begin{align*}
        \sigma \sqrt{\frac{2 \log \frac{1}{\delta}}{n}} = \frac{\log \frac{1}{\delta}}{n} \left(\sqrt{3 C} - \frac{1}{2} + O\left(\frac{1}{\sqrt{C}} \right) \right)
    \end{align*}
    Then, by symmetry, the circumradius $R$ of the $\mu_j$ is
    \begin{align*}
        R &\ge \frac{\log \frac{1}{\delta}}{n} \left(\sqrt{3 C} - \frac{1}{3} + O\left(\frac{1}{C} \right) \right)\\
        &\ge \left(1 + \frac{1}{10 \sqrt{3 C}} \right)\sigma \sqrt{\frac{2 \log \frac{2}{\delta}}{n}} 
    \end{align*}
    So, for $\tau = \frac{1}{10 \sqrt{ 3 C}}$, we have the claim for this particular $\sigma^2$. Rescaling gives the claim for any $\sigma^2$.
\end{proof}

\subsection{Eric's scratch}
XXX

OK, so the above proof didn't work, but that example (one $k_{-}$, two $k_{+}$) had these properties.  Let $\sigma_j^2$ be the variance in direction $v_j$, and $\sigma_{\perp}^2$ be the variance perpendicular to it.  We have:
\begin{align*}
    \mu_j &= (\frac{\log \frac{1}{\delta}}{n}) (\sqrt{3C} - \frac{1}{3} + O(\frac{1}{C})) \cdot (-v_j)\\
    \sigma_{j}^2 &= (\frac{\log \frac{1}{\delta}}{2n}) (3C - \sqrt{3C} + 1 + O(\frac{1}{C}))\\
    \sigma_{\perp}^2 &= (\frac{\log \frac{1}{\delta}}{2n}) (3C + \sqrt{3C} + \frac{1}{3} + O(\frac{1}{C}))
\end{align*}

We could do the same thing but with one $k_+$ and two $k_{-}$; this ends up just flipping the $\sqrt{C}$ terms, getting the following:
\begin{align*}
    \mu_j &= (\frac{\log \frac{1}{\delta}}{n}) (\sqrt{3C} + \frac{1}{3} + O(\frac{1}{C})) \cdot (v_j)\\
    \sigma_{j}^2 &= (\frac{\log \frac{1}{\delta}}{2n}) (3C + \sqrt{3C} + 1 + O(\frac{1}{C}))\\
    \sigma_{\perp}^2 &= (\frac{\log \frac{1}{\delta}}{2n}) (3C - \sqrt{3C} + \frac{1}{3} + O(\frac{1}{C}))
\end{align*}

\paragraph{First attempt.} So now, as a first attempt, consider the "hexagon" produced by taking the second option, combined with the first option flipped 180 degrees.  This has a $\delta^2$ chance of observing $k$ in each of the $6$ directions, and has mean + variance just the sum of the previous two.  The $\sqrt{3C}$ terms cancel!  This gives

\begin{align*}
    \mu_j &= (\frac{\log \frac{1}{\delta^2}}{n}) ( \sqrt{3C} + O(\frac{1}{C})) \cdot v_j\\
    \sigma_{j}^2 &= (\frac{\log \frac{1}{\delta^2}}{2n}) (3C + 1 + O(\frac{1}{C}))\\
    \sigma_{\perp}^2 &= (\frac{\log \frac{1}{\delta^2}}{2n}) (3C  + \frac{1}{3} + O(\frac{1}{C}))
\end{align*}

which is just \emph{barely} not good enough:  for this $\delta^2$ probability event, we have
\[
\sqrt{2 \norm{\Sigma} \frac{\log \frac{1}{\delta^2}}{n}} = (\frac{\log \frac{1}{\delta^2}}{n}) (\sqrt{3C} + O(\frac{1}{\sqrt{C}})) \approx \mu_j.
\]
That is, it matches down to $O(1/\sqrt{C})$ terms.  But the $1/\sqrt{C}$ term is not in our favor.

\paragraph{Second attempt.} But the above is \emph{so close} to working.  Can we futz with it a bit to make it work?  Here's one attempt.

Rather than have the $(+,-,-)$ option be simply the $(-,+,+)$ option flipped, what if we choose a different value for $C$, \emph{and} a different scale?  In particular, let's make the $(+,-,-)$ option have $C_+ = a C_{-}$, and place its points at $- b v_i$. We will end up setting $a = 1/b^4$, and $b = 1 + \eps$ for some small constant $\eps = \Theta(1/\sqrt{C})$.

Because $\sqrt{a}b^2 = 1$, the $(+,-,-)$ option now has mean and variances
\begin{align*}
    \mu_j &= (\frac{\log \frac{1}{\delta}}{n}) (\sqrt{3C a}b + \frac{b}{3} + O(\frac{1}{C})) \cdot (v_j)\\
    \sigma_{j}^2 &= (\frac{\log \frac{1}{\delta}}{2n}) (3Cab^2 + \sqrt{3Ca}b^2 + b^2 + O(\frac{1}{C}))\\
    \sigma_{\perp}^2 &= (\frac{\log \frac{1}{\delta}}{2n}) (3Cab^2 - \sqrt{3Ca}b^2 + \frac{b^2}{3} + O(\frac{1}{C})).
\end{align*}
Using that $\sqrt{a} = 1/b^2$, this is
\begin{align*}
    \mu_j &= (\frac{\log \frac{1}{\delta}}{n}) (\sqrt{3C}/b + \frac{b}{3} + O(\frac{1}{C})) \cdot (v_j)\\
    \sigma_{j}^2 &= (\frac{\log \frac{1}{\delta}}{2n}) (3C/b^2 + \sqrt{3C} + b^2 + O(\frac{1}{C}))\\
    \sigma_{\perp}^2 &= (\frac{\log \frac{1}{\delta}}{2n}) (3C/b^2 - \sqrt{3C} + \frac{b^2}{3} + O(\frac{1}{C})).
\end{align*}
so the combination still has the $\sqrt{3C}$ term in the variance cancel; the combination has mean and variances (switching to $\log \frac{1}{\delta^2}$ out front):
\begin{align*}
    \mu_j &= (\frac{\log \frac{1}{\delta^2}}{n}) ( \sqrt{3C}\frac{1 + 1/b}{2} + \frac{b-1}{6} + O(\frac{1}{C})) \cdot v_j\\
    \sigma_{j}^2 &= (\frac{\log \frac{1}{\delta^2}}{2n}) (3C\frac{1 + 1/b^2}{2} + 1 + O(\frac{1}{C}))\\
    \sigma_{\perp}^2 &= (\frac{\log \frac{1}{\delta^2}}{2n}) (3C\frac{1 + 1/b^2}{2}  + \frac{1}{3} + O(\frac{1}{C}))
\end{align*}
Setting $b = \frac{1}{1 - \eps} = 1 + \eps + O(\eps^2)$, we have
\begin{align*}
    \mu_j &= (\frac{\log \frac{1}{\delta^2}}{n}) ( \sqrt{3C}(1 - \eps/2) + \frac{\eps}{6} + O(\eps^2) + O(\frac{1}{C})) \cdot v_j\\
    \sigma_j^2, \sigma_{\perp}^2 &\leq (\frac{\log \frac{1}{\delta^2}}{2n}) (3C(1 -  \eps + \eps^2/2) + 1 + O(\frac{1}{C}))
\end{align*}
and so the tolerable error is
\[
\sqrt{2 \sigma^2 \frac{\log \frac{1}{\delta^2}}{n}} =  (\frac{\log \frac{1}{\delta^2}}{n}) (\sqrt{3C} (1 - \eps/2 + \eps^2/8) + O(\eps^3 \sqrt{C}) + \frac{1}{2 \sqrt{3C}} + O(\frac{1}{C} + \frac{\eps}{\sqrt{C}}))
\]
Set $\eps = \frac{\alpha}{\sqrt{C}}$ for a constant $\alpha$, unfortunately this doesn't work... the terms match until the $1/\sqrt{C}$ order, where $\mu$ has $\alpha/6$ and error tolerance has $\frac{1}{2\sqrt{3}} + \alpha^2/8$, but for no $\alpha$ is the former larger.


\paragraph{3rd attempt?}
I tried making the variance perfectly spherical with the above strategy, it's complicated to set $a$ and $b$ precisely but you can do it numerically, and it seems to still not work.

There's still a $\frac{0.225}{\sqrt{C}}$ gap.  (The above analysis instead gets like a $\frac{0.28}{\sqrt{C}}$ gap.)

\paragraph{4th approach} A completely different approach is:
 take the current example, which has a bit of slack in the covariance in the $v_j$ direction, and place $\eps \log(1/\delta)/n$ mass at a point far away in the $-v_j$ direction.  Place it such that the variance becomes spherical; now there's a $\delta^\eps$ chance that the added point isn't seen, while the mean is shifted slightly further in the $-v_j$ direction.
 
but some calculation suggests that this improves the situation from the current ($\sqrt{3C} - 1/3$ mean, error bound of $\sqrt{3C} + 1/2$ to ($\sqrt{3C} + 1/6$ mean, error bound of $\sqrt{3C} + 1/2$)

so slightly better, but not good enough..  the problem is that this "invisible" point is not a very efficient use of covariance.

More carefully: in the $(-,+,+)$ example there is $\sqrt{3C} \log \frac{1}{\delta} / n$  ``free" variance in the $v_j$ direction.
Suppose we place a $\eps \log \frac{1}{\delta}/n$ mass at $(\sqrt{3 C}/\eps)^{1/2} \cdot (-v_j)$.  There is a $\delta^{\eps}$ chance you won't see it.  It gives variance matching our free variance.  It shifts the mean by $(\sqrt{3C} \eps)^{1/2} \frac{\log \frac{1}{\delta}}{n}$.  So then we have
\begin{align*}
    \mu &= \frac{\log \frac{1}{\delta}}{n} (\sqrt{3C} - \frac{1}{3} + (\sqrt{3C}\eps)^{1/2})\\
    \sigma^2 &= \frac{\log \frac{1}{\delta}}{2n} (3C + \sqrt{3C} + 1/3) \approx \frac{\log \frac{1}{\delta}}{2n} (\sqrt{3C} + \frac{1}{2})^2
\end{align*}
but now we have a $\delta^{1+\eps}$ chance of seeing $(k,k,k,0)$ so we need to change the leading term to that:
\begin{align*}
    \mu &\approx \frac{\log \frac{1}{\delta^{1+\eps}}}{n} (\sqrt{3C} - \frac{1}{3} + (\sqrt{3C}\eps)^{1/2} - \eps \sqrt{3C})\\
    \sigma^2 &\approx \frac{\log \frac{1}{\delta^{1+\eps}}}{2n} (\sqrt{3C} + \frac{1}{2} - \sqrt{3C}\eps/2)^2
\end{align*}

Setting $a^2 = \sqrt{3C}\eps$, this is
\begin{align*}
    \mu &\approx \frac{\log \frac{1}{\delta^{1+\eps}}}{n} (\sqrt{3C} - \frac{1}{3} + a - a^2)\\
    \sigma^2 &\approx \frac{\log \frac{1}{\delta^{1+\eps}}}{2n} (\sqrt{3C} + \frac{1}{2} - a^2/2)^2
\end{align*}
the difference is $-\frac{5}{6} - \frac{a^2}{2} + a$, which is maximized at $a=1$, it is still $-\frac{1}{3}$ so the gap remains.

(Unlike the hexagon, the gap remains \emph{constant} not just $1/\sqrt{C}$.)

\paragraph{5th attempt.}  I guess we could go back to the hexagon, but adjust the $\delta$ somehow?  The current analysis effectively sets $\log \delta_i$ to the same $\frac{1}{3} \log \frac{1}{\delta}$ for the two directions, and $\frac{1}{12} \log \frac{1}{\delta}$ for the 4 off-axis directions; maybe there's some slack from varying that so the two triangles don't each get the same $\sqrt{\delta}$?  We could change that $\alpha$, AND the scale, AND the $C$.  None will likely change much, but conceivably enough order-$1/\sqrt{C}$ shifts will give us a win.  Even for the single triangle, varying $\alpha$ seemed to give a $\Theta(1/\sqrt{C})$ improvement to $\mu - \sigma$.
It's not worth it for the triangle where you needed $\Omega(1)$ improvement, but for the hexagon?  Conceivable.

$(+,-,-)$ gives for $\alpha = \frac{2}{3} + \eps$,

\begin{align*}
    \mu &= \frac{\log \frac{1}{\delta}}{n} (\sqrt{3C}(\frac{\sqrt{4 + 6 \eps} + \sqrt{1 - 3\eps}}{3}) + \frac{1}{3} + O(1/C))\\
    \sigma_j^2 &\approx \frac{\log \frac{1}{\delta}}{2n} (3C + \sqrt{3C} (\frac{2 \sqrt{4 + 6 \eps} - \sqrt{1-3\eps}}{3}) + 1 + \eps)\\
    \sigma_{\perp}^2 &\approx \frac{\log \frac{1}{\delta}}{2n} (3C - \sqrt{3C} (\frac{2 \sqrt{4 + 6 \eps} - \sqrt{1-3\eps}}{3}) + \frac{1}{3} - \eps)
\end{align*}
while I think $(-,+,+)$ should give
\begin{align*}
    \mu &= \frac{\log \frac{1}{\delta}}{n} (\sqrt{3C}(\frac{\sqrt{4 + 6 \eps} + \sqrt{1 - 3\eps}}{3}) - \frac{1}{3} + O(1/C))\\
    \sigma_j^2 &\approx \frac{\log \frac{1}{\delta}}{2n} (3C - \sqrt{3C} (\frac{2 \sqrt{4 + 6 \eps} - \sqrt{1-3\eps}}{3}) + 1 + \eps)\\
    \sigma_{\perp}^2 &\approx \frac{\log \frac{1}{\delta}}{2n} +(3C - \sqrt{3C} (\frac{2 \sqrt{4 + 6 \eps} - \sqrt{1-3\eps}}{3}) + \frac{1}{3} - \eps)
\end{align*}
so with an even mixture, the variance terms cancel regardless of $\eps$, and we just want to pick $\eps$ to maximize $\mu$, which is $\eps = 0$.

One could imagine combining with the scale change, but that seems unlikely to help much?  The scale change is already a lower order term, so the benefit would be at most second order.

\paragraph{6th attempt.}

Going back to the first attempt, it was made with a 50-50 split of the two $\delta$; effectively, each triangle is given $\delta^{\frac{1}{2}}$ failure probability.  One could vary this, giving $\delta^{\frac{1}{2} \pm \eps}$ to the two triangles.

Some calculation suggests to me that this gives a $\Theta(\eps) - \Theta(\eps^2 \sqrt{C})$ improvement, which is up to $\Theta(\frac{1}{\sqrt{C}})$---so of the same order as the gap we're trying to cover.  I haven't done the calculation to see what constant we can get; it is possible that this improvement on its own, or (this improvement) + (2nd attempt's improvement) together, can overcome the gap.

\section{Shivam's calculation}
\paragraph{Attempt 6 alone.} Suppose we put $\delta^{1- \eps_1}$ probability on the first (one $k_-$, two $k_+$) triangle, and $\delta^{1 + \eps_1}$ on the second triangle. We will finally set $\eps_1 = \frac{\alpha_1}{\sqrt{C}}$ for some constant $\alpha_1$. We have
\begin{align*}
    \mu_j &= (\frac{\log \frac{1}{\delta^2}}{n} ) (\sqrt{3 C} + \frac{2 \eps_1}{3} + O\left(\frac{1}{C} \right)) \cdot v_j\\
    \sigma^2_j &= \left(\frac{\log \frac{1}{\delta^2}}{2n} \right) \left(3C + \sqrt{3 C}(2 \eps_1) + 1+ O\left(\frac{1}{C} \right)  \right)\\
    \sigma_\perp^2 &= \left(\frac{\log \frac{1}{\delta^2}}{2n} \right) \left(3C - \sqrt{3C} (2 \eps_1) + \frac{1}{3} + O\left(\frac{1}{C} \right) \right)
\end{align*}
Then, our error radius is
\begin{align*}
    \sqrt{2 \|\Sigma\| \frac{\log \frac{1}{\delta^2}}{n}} &= \left(\frac{\log \frac{1}{\delta^2}}{n} \right) \left(\sqrt{3 C} + \eps_1 +   \right)
\end{align*}

\paragraph{High dimensions?} Let's first try the $+, -, -, - \dots$ case. The correct setting of $\alpha$ here is $\frac{d}{d+1}$. Then, 
\begin{align*}
    \mu_j = \frac{\log \frac{1}{\delta}}{n} \left( \right)
\end{align*}
%$k = C \log \frac{1}{\delta}$. Note that $\lam_i = k \pm \sqrt{2 k \log \frac{1}{\delta}} + \frac{2}{3} \log \frac{1}{\delta}$. Let's again look at the $+,-,-$ and $-,+,+$ cases first. Recall that $\eps_i = \sqrt{2 k \log \frac{1}{\delta}}$, and we're assigning probability $\delta^{x_i}$ to vertex $i$. So, $x_2 = x_3 = \frac{1 - x_1}{2}$. Anyway, abstractly, the mean is
%\begin{align*}
%    &\mu_{+, -, -} = \left(k_1 + \eps_1 \sqrt{x_1} + \frac{2 x_1}{3} \log \frac{1}{\delta} \right) v_1 + \left(k_2 - \eps_2 \sqrt{x_2}
%    + \frac{2x_2}{3} \log \frac{1}{\delta} \right) v_2 \\
%        &+\left(k_3 - \eps_3 \sqrt{x_3} + \frac{2x_3}{3} \log \frac{1}{\delta} \right) v_3
%\end{align*}
%In the $k, k, k$ case,
%\begin{align*}
%    \mu_{+, -, -} &= \left(\eps_1 \sqrt{x_1} + \frac{\eps_2 \sqrt{x_2} + \eps_3 \sqrt{x_3}}{2} + \frac{2 x_1 - x_2 - x_3}{3} \log \frac{1}{\delta}\right) v_1\\
%    &=\left(\left(\sqrt{2 C} \left(\sqrt{x_1} + \sqrt{\frac{1 - x_1}{2}} \right) + \frac{3 x_1 - 1}{3} \right)\log \frac{1}{\delta} \right) v_1
%\end{align*}
%For $x_1 = 2/3$,
%\begin{align*}
%    \mu_{+, -, -} &= \left(\left(\sqrt{2 C}\left(\sqrt{\frac{2}{3}} + \sqrt{\frac{1}{6}} \right) + \frac{1}{3}\right) \log \frac{1}{\delta} \right) v_1\\
%    &= \left( \sqrt{3 C} + \frac{1}{3}\right)\log \frac{1}{\delta} v_1
%\end{align*}
%
%The covariance $\Sigma_{+, -, -}$ is
%\begin{align*}
%    &\Sigma_{+, -, -} = \left(k + \eps_1 \sqrt{x_1} + \frac{2x_1}{3} \log \frac{1}{\delta} \right) v_1 v_1^T + \left(k - \eps_2 \sqrt{x_2}
%    + \frac{2x_2}{3} \log \frac{1}{\delta} \right) v_2 v_2^T\\
%        &+\left(k - \eps_3 \sqrt{x_3} + \frac{2x_3}{3} \log \frac{1}{\delta} \right) v_3 v_3^T 
%\end{align*}
%so that
%\begin{align*}
%    \|\Sigma_{+,-,-}\| &= v_1^T \Sigma_{+,-,-} v_1 = \frac{3 C \log \frac{1}{\delta}}{2} + \eps_1 \sqrt{x_1} - \frac{\eps_2 \sqrt{x_2} + \eps_3 \sqrt{x_3}}{4} + \frac{2 x_1 + x_2/2 + x_3/2}{3} \log \frac{1}{\delta}\\
%    &= \left(\frac{3C}{2} + \sqrt{2 C} \left(\frac{2 \sqrt{x_1} - \sqrt{\frac{1 - x_1}{2}}}{2} \right) + \frac{2x_1 + x_2/2 + x_3/2 }{3}\right) \log \frac{1}{\delta}
%\end{align*}
%For $x_1 = 2/3$,
%\begin{align*}
%    \|\Sigma_{+,-,-}\| = \left(\frac{3C}{2} + \frac{\sqrt{3 C}}{2} + \frac{1}{2} \right)\log \frac{1}{\delta}
%\end{align*}
%
%so that
%\begin{align*}
%    \sqrt{2 \|\Sigma_{+, -, -}\| \log \frac{1}{\delta}} &= \sqrt{3 C + \sqrt{3 C} + 1} \cdot \log \frac{1}{\delta}\\
%    &=\sqrt{3 C}\cdot \sqrt{1 + \frac{1}{\sqrt{3C}} + \frac{1}{3C}} \log \frac{1}{\delta}\\
%    &= \left(\sqrt{3C} + \frac{1}{2} + O(1/\sqrt{C}) \right) \log \frac{1}{\delta}
%\end{align*}
%
%So, we have that our output $\hat \mu$ must satisfy
%\begin{align*}
%    \|\hat \mu - \left(\sqrt{3 C} + \frac{1}{3} \right) \log \frac{1}{\delta} \cdot v_1\| \le \left(\sqrt{3C} + \frac{1}{2} + O(1/\sqrt{C}) \right) \log \frac{1}{\delta}
%\end{align*}
%Similarly, for $x_1 = 2/3$
%\begin{align*}
%    \mu_{-, +, +} = \left(- \sqrt{3C} + \frac{1}{3} \right) \log \frac{1}{\delta}
%\end{align*}
%and
%\begin{align*}
%      \|\Sigma_{-, +,+} \| = \left(\frac{3C}{2} - \frac{\sqrt{3C}}{2} + \frac{1}{2} \right)\log \frac{1}{\delta}
%\end{align*}
%so that
%\begin{align*}
%    \sqrt{2 \|\Sigma_{-, +, +}\| \log \frac{1}{\delta}} = \left(\sqrt{3C } - \frac{1}{2} + O(1/\sqrt{C}) \right) \log \frac{1}{\delta}
%\end{align*}
%So,
%\begin{align*}
%    \|\hat \mu - \left(-\sqrt{3 C} + \frac{1}{3} \right) \log \frac{1}{\delta} \cdot v_1\| \le \left(\sqrt{3C} - \frac{1}{2} + O(1/\sqrt{C}) \right) \log \frac{1}{\delta}
%\end{align*}
%That is, the intersection of the above two circles is at $\left(-\frac{1}{6}\log \frac{1}{\delta} + O(1/\sqrt{C}) \right)\cdot v_1$. But by symmetry, you have the same thing for $v_2$ and $v_3$. So there is a lower bound.
%So, for $k, k,k$, you must output $$

==> norm_talagrand.tex <==
\section{Norm deviation bounds using Talagrand's Inequality for empirical processes}

\begin{theorem}[Talagrand's inequality \cite{Talagrand1996NewCI, bousquet_subadditive}]
\label{thm:talagrand_bernstein_type}
    Let $X_1, \dots, X_n$ be independent $\chi$-valued random variables. Let $\F$ be a countable family of measurable real-valued functions on $\chi$ such that $\|f\|_\infty \le U \le \infty$ and $\E[f(X_1)] = \dots = \E[f(X_n)] = 0$ for all $f \in \F$. Let
    \[
    Z = \sup_{f \in \F} \sum_{i=1}^n f(X_i)
    \quad
    \text{or}
    \quad
    Z = \sup_{f \in \F} \left|\sum_{i=1}^n f(X_i) \right|
    \]
    Let 
    \[
    U^2 \ge \sigma^2 \ge \frac{1}{n} \sum_{i=1}^n \sup_{f \in \F}\E[f^2(X_i)]
    \quad
    \text{and}
    \quad
    \nu_n = 2U \E[Z] + n \sigma^2
    \]
    Then, for all $t \ge 0$,
    $$\Pr[Z \ge \E[Z] + t] \le \exp\left(\frac{- t^2}{2 \nu_n + 2 t U/3}\right)$$
\end{theorem}

\begin{theorem}[Direction-by-direction to norm concentration for Bernstein-type vectors]
    Suppose we have i.i.d. random variables $X_1, \dots, X_n \in \R^d$ with $\mu = \E[X_i]$ and $\Sigma \succcurlyeq \text{Cov}(X_i)$ such that for every $v \in \R^d, \|v\| = 1$, $v^T(X_i - \mu) \le c$.
    Then, we have that with probability $1 - \delta$,
    $$\left\|\frac{1}{n} \sum_{i=1}^n X_i - \mu \right\| \le \sqrt{\frac{\tr(\Sigma)}{n}} + \sqrt{\|\Sigma\| + (2c) \sqrt{\frac{\tr(\Sigma)}{n}}} \sqrt{\frac{2 \log \frac{1}{\delta}}{n}} + \frac{2 c \log \frac{1}{\delta}}{3 n}$$
\end{theorem}
\begin{proof}
    Note that we cannot directly apply Theorem~\ref{thm:talagrand_bernstein_type}  since it requires a \emph{countable} family of functions. Instead, we will proceed by a net argument.
    
    For $\eps > 0$, let $\mathcal N_\eps = \{v_1, \dots, v_{|\mathcal N_\eps|}\}$ be an $\eps$-net of $S^{n-1}$, so that for any $x \in S^{n-1}$, $\min_{v \in \mathcal N_\eps} \|x - v\| \le \eps$. Let $\F_\eps = \{f(X) = v^T X | v \in \mathcal N_\eps\}$. 
    First, 
    \begin{align*}
    \E\left[\sup_{v \in \mathcal N_\eps} v^T \left( \frac{1}{n} \sum_{i=1}^n X_i - \mu\right)\right] &\le \E\left[ \sup_{v \in S^{n-1}} v^T \left( \frac{1}{n} \sum_{i=1}^n X_i - \mu \right)\right]\\
    &= \E\left[\left\|\frac{1}{n} \sum_{i=1}^n X_i - \mu \right\| \right]\\
    &\le \sqrt{\E\left[\left\|\frac{1}{n} \sum_{i=1}^n X_i - \mu \right\|^2 \right]}\\
    &= \sqrt{\frac{\tr(\Sigma)}{n}}
    \end{align*}
    So, applying Theorem~\ref{thm:talagrand_bernstein_type} yields that with probability $1 - \delta$,
    $$\sup_{v \in \mathcal N_\eps} v^T \left(\sum_{i=1}^n \frac{1}{n} X_i - \mu\right) \le \sqrt{\frac{\tr(\Sigma)}{n}} + \sqrt{\|\Sigma\| + (2 c) \sqrt{\frac{\tr(\Sigma)}{n}}} \sqrt{\frac{2 \log \frac{1}{\delta}}{n}} + \frac{2 c \log \frac{1}{\delta}}{3 n}$$
    Now,
    \begin{align*}
        \left\|\frac{1}{n}\sum_{i=1}^n X_i - \mu \right\| &= \sup_{v \in S^{n-1}} v^T \left(\frac{1}{n} \sum_{i=1}^n X_i - \mu \right)\\
        &\le \sup_{z \in \eps S^{n-1}} z^T \left(\frac{1}{n} \sum_{i=1}^n X_i - \mu \right) + \sup_{v \in \mathcal N_\eps} v^T \left(\frac{1}{n} \sum_{i=1}^n X_i - \mu \right)\\
        &\le \eps \left\|\frac{1}{n} \sum_{i=1}^n X_i - \mu\right\| + \sup_{v \in \mathcal N_\eps} \left(\frac{1}{n} \sum_{i=1}^n X_i - \mu \right)
    \end{align*}
    Sending $\eps \to 0$ gives the claim
\end{proof}

%\section{New approach}
%\begin{lemma}
%    Let $X \in \R^d$ be a random variable such that for every $v \in S^{d-1}$, and $\lam \ge 0$, $$\E_X[\exp(\lam (v^T X))] \le \exp(\lam^2/2) $$
%    Then, for $\delta = e^{-o(d)}$, we have that with probability $1 - \delta$,
%    $$\|X\| \le \sqrt{d} + (1+o(1))\sqrt{2\log(1/\delta)}$$
%\end{lemma}
%
%\begin{proof}
%    Let $\gamma > 0$, and suppose, for the sake of contradiction, that with probability greater than $\delta + \gamma$,
%    $$\|X\| > \sqrt{d} + \sqrt{2 \log(1/\delta)}$$
%    Then, we will pick a random direction $v \in S^{d-1}$, and lower bound the probability that $v^T X > \sqrt{2 \log \frac{1}{\delta}}$. By symmetry, we have that for a random direction $v \sim S^{d-1}$, $v^T X = \|X\| v^T e_1$. So, 
%    \begin{align*}
%        \Pr_{X, v \sim S^{d-1}} \left[v^T X > \sqrt{2 \log \frac{1}{\delta}} \right] &= \Pr_{X, v \sim S^{d-1}} \left[\|X\| v^T e_1 > \sqrt{ 2 \log \frac{1}{\delta}} \right]\\
%        &= \Pr_{X, w \sim \mathcal N\left(0,\frac{1}{d}I_{d \times d}\right) }\left[\|X\| \frac{w^T e_1}{\|w\|} > \sqrt{2 \log \frac{1}{\delta}}\right]
%    \end{align*}
%    Now, since $w \sim \mathcal N\left(0, \frac{1}{d}I_{d \times d} \right)$, we have that $\|w\|^2 \sim \chi^2_d/d$. So, with probability at least $1 - e^{-\Omega(d)}$, $$\|w\| \ge 0.99$$
%    %so that
%    %$$\|w\| \ge 1 -  \Omega\left(\sqrt{\frac{1}{d} \log \frac{1}{\beta}}\right)$$
%    So, using this and our assumption,
%    \begin{align*}
%        &\Pr_{X, v \sim S^{d-1}} \left[v^T X > \sqrt{2 \log \frac{1}{\delta}} \right]\\
%        &> (\delta + \gamma)(1 - e^{-\Omega(d)}) \Pr_{w \sim \mathcal N(0, \frac{1}{d} I_{d \times d})} \left[\left(\sqrt{d} + \sqrt{2 \log \frac{1}{\delta}} \right) \frac{w^T e_1}{0.99} > \sqrt{2 \log \frac{1}{\delta}}  \right]\\
%        &\ge (\delta + \gamma)(1 - e^{-\Omega(d)}) \Pr_{u \sim \mathcal N(0, \frac{1}{d})}\left[\left(\sqrt{d} + \sqrt{2 \log \frac{1}{\delta}}  \right) u> \sqrt{2 \log \frac{1}{\delta}} \right]\\
%        %&= (\delta + \gamma) (1 - \beta) \Pr_{u \sim \mathcal N(0, \frac{1}{d})}\left[\left(\sqrt{d} + \sqrt{2 \log \frac{1}{\delta}} \right) u > \sqrt{2 \log \frac{1}{\delta}}-  \Omega\left( \sqrt{\frac{1}{d} \log \frac{1}{\delta} \log \frac{1}{\beta}} \right)\right]\\
%        &\ge (\delta + \gamma) (1 - e^{-\Omega( d)}) \Pr_{y \sim \mathcal N\left(0, 1 + \frac{2 \log \frac{1}{\delta}}{d}\right)}\left[ y > \sqrt{2 \log \frac{1}{\delta}} \right]\\
%        &\ge (\delta + \gamma)(1 - e^{-\Omega(d)})^2\\
%    \end{align*}
%    So, there is a setting of $\gamma = e^{-\Omega(d)}$ such that for any $\delta = e^{-o(d)}$,
%    $$\Pr_{X, v \sim S^{d-1}}\left[ v^T X > \sqrt{2 \log \frac{1}{\delta}}\right] > \delta$$
%    But this means that there exists a $v_* \in S^{d-1}$ such that
%    $$\Pr_X\left[v_*^T X > \sqrt{2 \log \frac{1}{\delta}} \right] >\delta$$
%    which contradicts our assumption that \emph{for all} $v \in S^{d-1}$ and $\lam \ge 0$,
%    $$\E_X\left[\exp(\lam(v^T X)) \right] \le \exp(\lam^2/2)$$
%    So, we have shown that with probability at least $1 - \delta - \gamma$,
%    $$\|X\| \le \sqrt{d} + \sqrt{2 \log(1/\delta)}$$
%    Letting $\delta' = \delta + \gamma = \delta(1+o(1))$, we have that with probability $1 - \delta'$,
%    $$\|X\| \le \sqrt{d} + \sqrt{2 \log(1/\delta')} \le \sqrt{d} + (1+o(1)) \sqrt{2 \log \frac{1}{\delta'}}$$
%    
%\end{proof}
%
%\begin{lemma}
%    Let $X \in \R^d$ be a random variable such that for every $v \in S^{d-1}$, and $\lam \ge 0$, $$\E_X[\exp(\lam (v^T X))] \le \exp\left(\frac{\lam^2}{2} (v^T \Sigma v)\right) $$
%    Then, for $\delta = e^{-o(d)}$, we have that with probability $1 - \delta$,
%    $$\|X\| \le \sqrt{\tr(\Sigma)} + (1+o(1))\sqrt{2\|\Sigma\|\log(1/\delta)}$$
%\end{lemma}
%
%\begin{proof}
%        Let $\gamma > 0$, and suppose, for the sake of contradiction, that with probability greater than $\delta + \gamma$,
%    $$\|X\| > \sqrt{\tr(\Sigma)} + \sqrt{2\|\Sigma\| \log(1/\delta)}$$
%    Then, we will pick a random direction $v \in S^{d-1}$, and lower bound the probability that $v^T \Sigma^{-1/2}X > \sqrt{2 \log \frac{1}{\delta}}$. By symmetry, we have that for a random direction $v \sim S^{d-1}$, $v^T X = \|X\| v^T e_1$. So, 
%    \begin{align*}
%        \Pr_{X, v \sim S^{d-1}} \left[v^T X > \sqrt{2 \log \frac{1}{\delta}} \right] &= \Pr_{X, v \sim S^{d-1}} \left[\|X\| v^T e_1 > \sqrt{ 2 \log \frac{1}{\delta}} \right]\\
%        &= \Pr_{X, w \sim \mathcal N\left(0,\frac{1}{d}I_{d \times d}\right) }\left[\|X\| \frac{w^T e_1}{\|w\|} > \sqrt{2 \log \frac{1}{\delta}}\right]
%    \end{align*}
%    Now, since $w \sim \mathcal N\left(0, \frac{1}{d}I_{d \times d} \right)$, we have that $\|w\|^2 \sim \chi^2_d/d$. So, with probability at least $1 - e^{-\Omega(d)}$, $$\|w\| \ge 0.99$$
%    %so that
%    %$$\|w\| \ge 1 -  \Omega\left(\sqrt{\frac{1}{d} \log \frac{1}{\beta}}\right)$$
%    So, using this and our assumption,
%    \begin{align*}
%        &\Pr_{X, v \sim S^{d-1}} \left[v^T X > \sqrt{2 \log \frac{1}{\delta}} \right]\\
%        &> (\delta + \gamma)(1 - e^{-\Omega(d)}) \Pr_{w \sim \mathcal N(0, \frac{1}{d} I_{d \times d})} \left[\left(\sqrt{d} + \sqrt{2 \log \frac{1}{\delta}} \right) \frac{w^T e_1}{0.99} > \sqrt{2 \log \frac{1}{\delta}}  \right]\\
%        &\ge (\delta + \gamma)(1 - e^{-\Omega(d)}) \Pr_{u \sim \mathcal N(0, \frac{1}{d})}\left[\left(\sqrt{d} + \sqrt{2 \log \frac{1}{\delta}}  \right) u> \sqrt{2 \log \frac{1}{\delta}} \right]\\
%        %&= (\delta + \gamma) (1 - \beta) \Pr_{u \sim \mathcal N(0, \frac{1}{d})}\left[\left(\sqrt{d} + \sqrt{2 \log \frac{1}{\delta}} \right) u > \sqrt{2 \log \frac{1}{\delta}}-  \Omega\left( \sqrt{\frac{1}{d} \log \frac{1}{\delta} \log \frac{1}{\beta}} \right)\right]\\
%        &\ge (\delta + \gamma) (1 - e^{-\Omega( d)}) \Pr_{y \sim \mathcal N\left(0, 1 + \frac{2 \log \frac{1}{\delta}}{d}\right)}\left[ y > \sqrt{2 \log \frac{1}{\delta}} \right]\\
%        &\ge (\delta + \gamma)(1 - e^{-\Omega(d)})^2\\
%    \end{align*}
%    So, there is a setting of $\gamma = e^{-\Omega(d)}$ such that for any $\delta = e^{-o(d)}$,
%    $$\Pr_{X, v \sim S^{d-1}}\left[ v^T X > \sqrt{2 \log \frac{1}{\delta}}\right] > \delta$$
%    But this means that there exists a $v_* \in S^{d-1}$ such that
%    $$\Pr_X\left[v_*^T X > \sqrt{2 \log \frac{1}{\delta}} \right] >\delta$$
%    which contradicts our assumption that \emph{for all} $v \in S^{d-1}$ and $\lam \ge 0$,
%    $$\E_X\left[\exp(\lam(v^T X)) \right] \le \exp(\lam^2/2)$$
%    So, we have shown that with probability at least $1 - \delta - \gamma$,
%    $$\|X\| \le \sqrt{d} + \sqrt{2 \log(1/\delta)}$$
%    Letting $\delta' = \delta + \gamma = \delta(1+o(1))$, we have that with probability $1 - \delta'$,
%    $$\|X\| \le \sqrt{d} + \sqrt{2 \log(1/\delta')} \le \sqrt{d} + (1+o(1)) \sqrt{2 \log \frac{1}{\delta'}}$$
%    
%\end{proof}
%

==> scratch.tex <==
\section{Scratch}

\begin{algorithm}[H]\caption{One-dimensional Mean Estimation of Non-negative variable when Higher Moments infinite}
    \label{alg:one_dim_finite_mean_infinite_moments} 
    %\vspace*{3mm}
    \paragraph{Input parameters:}
    \begin{itemize}
        \item Failure probability $\delta$, One-dimensional iid samples $x_1, \dots, x_n$.
    \end{itemize}
    \begin{enumerate}
        \item Remove the $2 \log \frac{1}{\delta}$ largest samples, and let the remaining samples be given by the set $S$.
        \item Return $\wh \mu$, the empirical mean of the samples in $S$.
    \end{enumerate}
\end{algorithm}

\begin{lemma}
    Consider any non-negative random variable $X$ over $\R$ with finite mean $\mu$. Given $n$ samples $x_1, \dots, x_n \sim X$, we have that the output $\wh \mu$ of Algorithm~\ref{alg:one_dim_finite_mean_infinite_moments} satisfies, with probability $1 - \delta$,
    \begin{align*}
        \frac{\wt \mu}{10} \le \wh \mu \le O(\mu)
    \end{align*}
    where $\wt \mu = \E\left[X \cdot 1_{\{X \le F^{-1}\left( 1 - \frac{16 \log \frac{1}{\delta}}{n} \right) \}} \right]$ for the CDF $F$ of $X$.
\end{lemma}
\begin{proof}
    By Markov's inequality,
    \begin{align*}
        \Pr\left[X \ge \frac{4 \mu n}{\log \frac{1}{\delta}} \right] \le \frac{\log \frac{1}{\delta}}{4 n}
    \end{align*}
    Let $E$ be the event that more than $2 \log \frac{1}{\delta}$ of the samples $x_1, \dots, x_n$ are larger than $\frac{4 \mu n}{\log \frac{1}{\delta}}$. We have, by Chernoff bound,
    \begin{align*}
        \Pr\left[E \right] \le \delta/10
    \end{align*}
    Moreover, conditioned on $\Bar E$, for the set $S$ as defined in Algorithm~\ref{alg:one_dim_finite_mean_infinite_moments}, we know that
    \begin{align*}
        \sum_{i \in S} x_i \le \sum_{i=1}^n x_i \cdot 1_{\{x_i \le \frac{4\mu n}{\log \frac{1}{\delta}}\}}
    \end{align*}
    Now, 
    \begin{align*}
        \E\left[x_i^2 \cdot 1_{\{x_i \le \frac{4\mu n}{\log \frac{1}{\delta}}\}} \right] \le \frac{4\mu^2 n}{\log \frac{1}{\delta}}
    \end{align*}
    So, by Bernstein's inequality, with probability $1 - \delta/4$,
    \begin{align*}
        \frac{1}{n} \sum_{i=1}^n x_i \cdot 1_{\{x_i \le \frac{4 \mu n}{\log \frac{1}{\delta}} \}} \lesssim \mu
    \end{align*}
    So, with probability $1 - \delta/2$,
    \begin{align*}
        \wh \mu \lesssim \mu
    \end{align*}
For the lower bound, consider the random variable $Y = X \cdot 1_{\{X \le F^{-1} \left(1 - \frac{16\log \frac{1}{\delta}}{n} \right)\}}$ so that $\wt \mu = \E[Y]$.

By Markov's inequality,
\begin{align*}
    \Pr\left[Y \ge  \frac{\wt \mu n}{6 \log \frac{1}{\delta}} \right] \le \frac{6\log \frac{1}{\delta}}{n}
\end{align*}
so that
\begin{align*}
    \E\left[ Y \cdot 1_{\{Y \le \frac{\wt \mu n}{6 \log \frac{1}{\delta}} \}}\right] + \frac{6 \log \frac{1}{\delta}}{n} \cdot F^{-1} \left(1 - \frac{16 \log \frac{1}{\delta}}{n} \right) \ge \E[Y] = \wt \mu
\end{align*}
since $Y \le F^{-1}\left(1 - \frac{16 \log \frac{1}{\delta}}{n} \right)$ by definition.


Let $E'$ be the event that one of the $8 \log \frac{1}{\delta}$ of the largest samples $x_1, \dots, x_n$ is smaller than $F^{-1} \left(1 - \frac{16 \log \frac{1}{\delta}}{n} \right)$. By the Chernoff bound,
\begin{align*}
    \Pr[E'] \le \delta/10
\end{align*}
Also,
\begin{align*}
    \E\left[Y^2 1_{\{Y \le \frac{ \wt \mu n}{6\log \frac{1}{\delta}}\}}\right] \le \frac{ \wt \mu^2 n}{6 \log \frac{1}{\delta}}
\end{align*}
So, by Bernstein's inequality, since the above shows that $x_i \cdot 1_{\{ x_i \le \frac{6\wt \mu n}{\log \frac{1}{\delta}}\}}$ has variance at most $\frac{\wt \mu^2 n}{6 \log \frac{1}{\delta}}$, and it is bounded by $\frac{\wt \mu n}{6 \log \frac{1}{\delta}}$, we have with probability $1 - \delta/4$,
\begin{align*}
    \frac{1}{n} \sum_{i=1}^n x_i \cdot 1_{\{x_i \le \frac{\wt \mu n}{6 \log \frac{1}{\delta}}\}} \ge \E\left[Y \cdot 1_{Y \le \frac{\wt \mu n}{6 \log \frac{1}{\delta}}} \right] - \frac{9\wt \mu}{10}
\end{align*}

So, under $\Bar E'$, since at least $6 \log \frac{1}{\delta}$ samples $x_i \in S$ are larger than $F^{-1} \left( 1 - \frac{16 \log \frac{1}{\delta}}{n}\right)$, and by the above, with probability $1 - \delta/2$ in total, we have
\begin{align*}
    \wh \mu &= \frac{1}{n} \sum_{i \in S} x_i \\
    &\ge \frac{1}{n} \sum_{i=1}^n x_i \cdot 1_{x_i \le \frac{\wt \mu n}{6 \log \frac{1}{\delta}}} + \frac{6 \log \frac{1}{\delta}}{n} \cdot F^{-1}\left(1 - \frac{16 \log \frac{1}{\delta}}{n} \right)\\
    &\ge \E\left[Y \cdot 1_{Y \le \frac{\wt \mu n}{6 \log \frac{1}{\delta}} } \right] + \frac{6 \log \frac{1}{\delta}}{n} \cdot F^{-1}\left(1 - \frac{16 \log \frac{1}{\delta}}{n} \right) - \frac{9 \wt \mu}{10}\\
    &\ge \frac{\wt \mu}{10}
\end{align*}
A union bound gives the claim.
%XXX Eric suggests: Bernstein says ifm mean $\mu$, range $[0, B]$ then $\sigma^2 \lesssim \mu B$ and
%\[
%\wh{\mu} \geq \mu - \sqrt{\mu B \frac{\log \frac{1}{\delta}}{n}}
%\]
%with probability $1-\delta$.  On the other hand, having at least $3 \log \frac{1}{\delta}$ values above $B$ means mean at least $B \frac{\log \frac{1}{\delta}}{n}$, giving:
%\[
%\max(\mu - \sqrt{\mu B \frac{\log \frac{1}{\delta}}{n}}, B \frac{\log \frac{1}{\delta}}{n}) \gtrsim \mu
%\]
%because it's like $\mu \max(1 - \sqrt{a}, a)$ for $a = \frac{B \log \frac{1}{\delta}}{n \mu}$.

\end{proof}

\subsection{Computing ``Robust Covariance''}
Our goal is to compute a matrix $\wh \Sigma$ such that for every direction $v$, $\frac{\wt \sigma_v}{100} \le v^T \wh \Sigma v \le O\left(v^T \Sigma v \right)$.
Here $\wt \sigma_v = 
